On the generic degree of two-parameter period mappings

We present a method for computing the generic degree of a period map defined on a quasi-projective surface. As an application, we explicitly compute the generic degree of three period maps underlying families of Calabi-Yau 3-folds coming from toric hypersurfaces. As a consequence, we show that the generic Torelli theorem holds for these cases.

==> 5star-copyComputation.tex <==

% ---------------------------------------
\section{Examples: Calabi-Yau 3-folds in toric variety}\label{sec4}
%----------------------------------------

In this section, we will calculate the degree of the period maps of type (1,2,2,1) that arise from the tautological family of Calabi-Yau hypersurface inside the toric variety over the simplified moduli. In other words, we will calculate
the degree of the map
\[
\Phi_{\mathrm{simp}}:\cM_{\mathrm{simp}}\rightarrow \mathrm{\Gamma}\backslash D,
\]
Moreover, 


The subsections will be named after the Hodge type of the Calabi-Yau 3-folds, namely in subsection $V_{(a,b)}$, we will study a Calabi-Yau 3-fold with Hodge numbers $(h^{2,1},h^{1,1}) = (a,b)$.


% ---------------------------------------

\subsection{$V_{(2,29)}$}
We study the smooth Calabi-Yau 3-folds $V$ with Hodge numbers $(h^{2,1},h^{1,1}) = (2,29)$, which is the anti-canonical hypersurface of the toric variety $X_{\Sigma^\circ}\cong \bP_{\Delta^\circ}$. The toric data for $\Delta^\circ$ and $\Sigma$ is
\begin{equation}\label{eqn5.1}
\begin{array}{c|cccccc}
\Xi&v_1 & v_2 & v_3 & v_4 & v_5 & v_6\\
\hline
r_1 & 1 & 0 & 0 & 0 & 1 & -2\\
r_2 & 0 & 1 & 0 & -1 & 1 & -1\\
r_3 & 0 & 0 & 1 & -1 & 2 & -2\\
r_4 & 0 & 0 & 0 & 0 & 3 & -3\\
\hline
w_1 & 1 & 0 & 0 & 0 & 1 & 1\\
w_2 & 0 & 1 & 1 & 1 & 0 & 0
\end{array}.
\end{equation}
The polytope $\Delta^\circ$ can be visualized as follows: $\Xi$ is naturally divided into two sets $\{v_1,v_5,v_6\}$ and $\{v_2,v_3,v_4\}$ where the points in both sets lie in the same plane, the 9 facets of $\Delta$ then come from choosing two points from each set.
After suspension, the toric data becomes
\begin{equation}\label{susfan5.2}
\begin{array}{c|ccccccc}
\bar\Xi& \bar v_1 & \bar v_2 & \bar v_3 &\bar  v_4 &\bar  v_5 &\bar  v_6 &\bar  v_7\\
\hline
\bar r_1 & 1 & 0 & 0 & 0 & 1 & -2 & 0\\
\bar r_2 & 0 & 1 & 0 & -1 & 1 & -1 & 0\\
\bar r_3 & 0 & 0 & 1 & -1 & 2 & -2 & 0\\
\bar r_4 & 0 & 0 & 0 & 0 & 3 & -3 & 0\\
\bar r_5 & 1 & 1 & 1 & 1 & 1 & 1 & 1\\
\hline
\bar w_1 & 1 & 0 & 0 & 0 & 1 & 1 & -3\\
\bar w_2 & 0 & 1 & 1 & 1 & 0 & 0 & -3
\end{array}.
\end{equation}


\subsubsection{Moduli spaces}\label{SubSec:4.1.1}
The toric data shows that $(\Delta^\circ \cap N)_0 = \Delta^\circ \cap N$, i.e., there is no integral point lies in the interior of codimension 2 face. Therefore, we have $\cM = \cM_{\mathrm{poly}}$.

From the multi-degree, it is clear that $\bP_{\Delta^\circ}$ has no root symmetry. Then the generic degree of the map $\phi:\cM_{\mathrm{poly}} \rightarrow  \cM_{\mathrm{simp}}$
is $|\tAut(\Sigma)/\tAut^{t}(\Sigma)|$, where $\tAut^{t}(\Sigma)$ is the normal subgroup of $\tAut(\Sigma)$ that acts trivially on $\cM_{\mathrm{poly}}$. 

Denote $\tAut(\Xi)$ as the subgroup of $\tAut(N)$ that permutes $\Xi$, then a direct calculation shows $\tAut(\Xi) = C_2\times C_3\rtimes S_3$, which acts on $\Xi$ as follows: the $C_2$ factor determines whether the permutation is even or odd, the set $\{v_2,v_3,v_4\}$ is sent to $\{v_2,v_3,v_4\}$ or $\{v_1,v_5,v_6\}$ respectively for the two cases. Then the $S_3$ factor determines the image of $v_2,v_3,v_4$ under the automorphism, and since the parity of the permutation is already determined, there are only $C_3$ choices for the image of $v_1,v_5,v_6$. From this description, it is also clear that every element in $\tAut(\Xi)$ permits the codimension-1 cones of $\Sigma$, thus we have
$\tAut(\Sigma) = \tAut(\Xi)$. As a subgroup of $S_6$ which acts on $\Xi$ by permutation, we have $\tAut(\Sigma)$ is generated by the permutations $a:= (234),b:=(34)(56),c:=(12)(35)(46)$. 






A generic point in $\bP(L(\Delta^\circ\cap N))$ is given by
\[
f = \lambda_1 t_1+\lambda_2t_2+\lambda_3t_3+\lambda_4 t^{-1}_2t_3^{-1}+\lambda_5t_1t_2t_3^2t_4^3+\lambda_6t_1^{-2}t_2^{-1}t_3^{-2}t_4^{-3}+\lambda_7,
\]
Then we have
\[
a\cdot f = \lambda_1 t_1+\lambda_3t_2+\lambda_4t_3+\lambda_2 t^{-1}_2t_3^{-1}+\lambda_5t_1t_2t_3^2t_4^3+\lambda_6t_1^{-2}t_2^{-1}t_3^{-2}t_4^{-3}+\lambda_7,
\]
which can be realized as a $T$-action 
\[
(t_1,t_2,t_3,t_4)\rightarrow (t_1,\lambda_2^{-1}\lambda_3t_2,\lambda_3^{-1}\lambda_4t_3,\lambda_2^{1/3}\lambda_3^{1/3}\lambda^{-2/3}_4t_4),
\]
similarly, $b$ can be realized as
\[
(t_1,t_2,t_3,t_4)\rightarrow (t_1,t_2,\lambda_3^{-1}\lambda_4t_3,\lambda_3^{2/3}\lambda^{-2/3}_4\lambda_5^{-1/3}\lambda_6^{1/3}t_4).
\]
However, $c$ can not be realized as a $T$-action, therefore, we have $\tAut^t(\Sigma) = C_3\rtimes S_3$, and the generic degree of $\phi$ is
\[
\deg_g(\phi)=|\tAut(\Sigma)/\tAut^t(\Sigma)|=2.
\]

The toric data for the secondary fan $\Sigma^s$ is
\begin{equation}
\begin{array}{c|ccc}
\Xi^s&v_1^s & v_2^s & v_3^s \\
\hline
r_1^s & 1 & 0 & -1 \\
r_2^s & 0 & 1 & -1 \\
\hline
w_1^s & 1 & 1 & 1 \\
\end{array}.
\end{equation}
Therefore, $\overline{\cM}_{\mathrm{simp}} = X_{\Sigma^s} \cong \bP^2 = \mathrm{Proj}\bC[Z_1,Z_2,Z_3]$, and the $\bZ/2\bZ$-action extend to $\overline{\cM}_{\mathrm{simp}}$ as $Z_1\leftrightarrow Z_2$ that ramifies at $Z_1=Z_2$.








\subsubsection{Picard-Fuchs system}\label{SubSec:4.1.2}
The GKZ ideal is generated by the Euler vectors $Z_i = \sum_{j=1}\bar v_{i,j}\delta_j - \beta_i$, $i=1,\dots,5$, $\beta_i = \delta_{i,5}$ and the toric ideal

The canonical affine chart is $\tSpec[z_1,z_2]$, with
\[
z_1 = \frac{\lambda_1\lambda_5\lambda_6}{\lambda_7^2},\quad z_2 = \frac{\lambda_2\lambda_3\lambda_4}{\lambda_7^2},
\]
then $D_{v_1^s} = \bV(z_1)$, $D_{v_{1^s}} = \bV(z_2)$. In the projective coordinates, this is the chart with $Z_3\neq 0$, and $z_i = \frac{X_i}{X_3}, i=1,2$.

The Picard-Fuchs ideal on $\cM$ is generated by the two differential operators
\begin{align*}
    & P_1:= \delta_1^3+z_1(3\delta_1+3\delta_2+1)(3\delta_1+3\delta_2+2)(3\delta_1+3\delta_2+3),\\
    & P_2:= (\delta_1^2-\delta_1\delta_2+\delta_2^2)+3(z_1+z_2)(3\delta_1+3\delta_2+1)(3\delta_1+3\delta_2+2).
\end{align*}
For simplicity, we rescale the local coordinates as $z_{1,2}':=3^3\cdot z_{1,2}$, and rename $z_{1,2}'$ as the new $z_{1,2}$. The Picard-Fuchs operators then become
\begin{equation}\label{eqp1p2}
\begin{aligned}
    & P_1:= \delta_1^3+z_1(\delta_1+\delta_2+\frac13)(\delta_1+\delta_2+\frac23)(\delta_1+\delta_2+1),\\
    & P_2:= (\delta_1^2-\delta_1\delta_2+\delta_2^2)+(z_1+z_2)(\delta_1+\delta_2+\frac13)(\delta_1+\delta_2+\frac23).
\end{aligned}
\end{equation}
The Picard-Fuchs ideal sheaf is denoted as $I$, which in the canonical affine affine chart is generated by $P_1$ and $P_2$. The associated $\cD$-module is clearly $\bZ/2\bZ$-equivariant under $z_1\leftrightarrow z_2$, $\partial_1\leftrightarrow \partial_2$.

%---------------------------------
\subsubsection{Discriminant locus}
%---------------------------------

The principal $A$-determinant $E_A$ is irreducible, and is thus equals to the $A$-discriminant $D_A$
\begin{align*}
D_A = & z_1^3 + 3z_1^2z_2 + 3z_1^2 + 3z_1z_2^2 - 21z_1z_2 + 3z_1 + z_2^3 + 3z_2^2 + 3z_2 + 1\\
 = & (z_1+z_2+1)^3-27z_1z_2
\end{align*}
so the discriminant locus is contained inside
\[
Disc= D_A\cup (\bar B\setminus B) = D_A\cup D_{v_1^s}\cup D_{v_2^s}\cup D_{v_3^s}.
\]

In the canonical affine chart $D_A$ intersect $D_{v_1^s}$ at $(-1,0)$ with 3-tangency, and by the $\bZ/2\bZ$ symmetry, $D_A$ intersect $D_{v_2^s}$ at $(0,-1)$ with 3-tangency.

In order to make $Disc$ only have normal crossing singularities, we need to blow-up these tangencies 3 times each. Since we will only be interested in the local monodromy, we only need to study the geometry at $z_1 = 0, z_2 = -1$. Denote the exceptional divisors of the three blow-ups as $E_1,E_2,E_3$, then we want to find 4 Picard-Fuchs ideals corresponding to the normal crossings 
\[
D_{v_1}\cap E_3, \quad E_1\cap E_2,\quad E_2\cap E_3\quad D_A\cap E_3,
\]
First, we make a change of coordinate of \eqref{eqp1p2} by $z_1 \rightarrow z_1$, $z_2\rightarrow z_2-1$. Then the local affine coordinates systems for each of the normal crossing is given by
\begin{equation*}
 \begin{aligned}
     & (s,t) = \left(\frac{z_1}{z_2^3},z_2\right),\quad && (s,t)= \left(\frac{z_2^2}{z_1},\frac{z_1}{z_2}\right),\\
     & (s,t)= \left(\frac{z_2^3}{z_1},\frac{z_1}{z_2^2}\right), \quad && (s,t) = \left(\frac{z_1}{z_2^3}-\frac{1}{27},z_2\right)
 \end{aligned}   
\end{equation*}
With $s=0$ gives the left divisor and $t=0$ gives the right divisor.


\subsubsection{Gauss-Manin connection and nilpotent cones}
By the local Torrelli theorem of Calabi-Yau manifolds, we can take a global multi-valued frame 
\begin{equation}\label{eqn:sympbasisV229}
w = (\Omega,\delta_1\Omega,\delta_2\Omega,\delta_1\delta_2\Omega,\delta_1^2\Omega,\delta_1^2\delta_2\Omega).
\end{equation}

The Gauss-Manin connection can be easily calculated from the Picard-Fuchs ideal by finding the 
\[
\begin{split}
&\nabla_{\delta_1} w =
w \left[
\begin{array}{rrrrrr}
     0 & 0 & 0 & 0 & z_1h^1_{15} & z_1h^1_{16} \\
     1 & 0 & 0 & 0 & z_1h^1_{25} & z_1h^1_{26}  \\
     0 & 0 & 0 & 0 & z_1h^1_{35} & z_1h^1_{36} \\
     0 & 0 & 1 & 0 & z_1h^1_{45} & z_1h^1_{46} \\
     0 & 1 & 0 & 0 & z_1h^1_{55} & z_1h^1_{56} \\
     0 & 0 & 0 & 1 & z_1h^1_{65} & z_1h^1_{66}
\end{array}
\right],\\
&\nabla_{\delta_2} w =
w \left[
\begin{array}{rrrrrr}
     0 & 0 & z_2h^2_{1,3} & z_2h^2_{1,4} & 0 & z_2h^2_{1,6}  \\
     0 & 0 & z_2h^2_{2,3} & z_2h^2_{2,4} & 0  & z_2h^2_{2,6} \\
     1 & 0 & z_2h^2_{3,3} & z_2h^2_{3,4} & 0 & z_2h^2_{3,6}  \\
     0 & 1 & 1+z_2h^2_{4,3} & z_2h^2_{4,4} & 0  & z_2h^2_{4,6} \\
     0 & 0 & -1 & z_2h^2_{4,4}& 0  & z_2h^2_{5,6} \\
     0 & 0 & 0 & 1+z_2h^2_{5,4} & 1 & z_2h^2_{6,6}
\end{array}
\right],
\end{split}
\]
 where $h^{i}_{lm}(z_1,z_2)$ are rational functions that is holomorphic at $z_1=z_2=0$. 

If we choose the base point $b\in\cM_{\mathrm{simp}}$ close to $z_1=z_2=0$, or more precisely, consider

\[
N_1 =\left[
\begin{array}{cccccc}
    0 & 0  & 0 & 0 & 0 & 0  \\ 
    1 & 0  & 0 & 0 & 0 & 0 \\ 
    0 & 0 &  0&  0&  0&  0\\ 
    0 & 0 & 1 & 0 & 0 & 0  \\ 
    0 & 1 & 0 & 0 & 0 & 0  \\ 
    0 & 0 & 0 & 1 & 0 &  0 \\ 
\end{array}
\right],\quad N_2 =\left[
\begin{array}{cccccc}
    0 & 0  & 0 & 0 & 0 & 0  \\ 
    0 & 0  & 0 & 0 & 0 & 0 \\ 
    1 & 0 &  0&  0&  0&  0\\ 
    0 & 1 & 1 & 0 & 0 & 0  \\ 
    0 & 0 & -1 & 0 & 0 & 0  \\ 
    0 & 0 & 0 & 1 & 1 &  0 \\ 
\end{array}
\right],
\]


\subsubsection{Local monodromy and LMHS type}
For any irreducible component of $D\subset\overline B\setminus B$, fix a local basis of $H^3(V_b,\bC)$, with $b$ near $D$. More precisely, we are taking a stalk of the nearby cycle sheaf on $D$ at $b\in D$. Then
we can define the local monodromy around $D$. Fix a local basis 



By the same method as in \cite{Chen23}, the types of LMHS of the rest possible two-dimensional nilpotent cones can be determined up to some ambiguity by calculating the Jordan normal form of the nilpotent operators of the boundary and using the polarization relations. The result is
\begin{align}
 \label{V229:cone1}    \mathrm{Cone}(D_{v_1^s},D_{v_2^s}) & = \braket{III_0|IV_2|III_0}\\
 \label{V229:cone2}   \mathrm{Cone}(D_{v_1^s},E_3) &  = \braket{III_0|IV_2|IV_1} \\ 
    \mathrm{Cone}(E_1,E_2) & = \braket{IV_1|IV_2(IV_1)|IV_1}\\
    \mathrm{Cone}(E_2,E_3) & = \braket{IV_1|IV_2(IV_1)|IV_1}\\
 \label{V229:cone5}    \mathrm{Cone}(D_A,E_3) & = \braket{I_1|IV_2|IV_1}
\end{align}
where there is another copy of cone \eqref{cone2}-\eqref{cone5} by the $\bZ_2$-symmetry of the $\cD$-module. The possible ambiguity has been indicated inside the parathesis. Since the monodromy around $D_{v_3^s}$ is finite, we have excluded the cones associated with it.


\subsubsection{Cohomology of $\bP_\Delta$}
Recall we have the correspondence between $\Xi$ and $T$-invariant divisors given by $v_i\leftrightarrow D_{v_i}$.  Further, recall $A_{3}(X_{\Sigma})$ is generated by the class of $T$-invariant divisors, so in what follows, we will use $D_{v_i}$ to denote either the $T$-invariant divisor, or its linear equivalence class or its cohomology class under Poincar{\'e} duality.
Associate to each $v_i$ a variable $x_i$ and consider the polynomial ring $\bZ[x_1,x_2,\cdots,x_6]$. Since $\bP_\Delta$ is smooth and complete, by Jurkiewicz-Danilov's theorem (see e.g. \cite{CLS11}), we have
$$
H^*(\bP_\Delta,\bZ) \cong \bZ[x_1,x_2\cdots,x_6]/(I_{RS}+J).
$$
The Stanley-Reisier ideal $I_{SR}$ is generated by the monomials $\prod_{i\in E}x_i$, as $E$ runs over all the subset of $\Delta$ such that $E$ does not form a cone in $\Sigma$. The Stanley-Reisier ideal 
can be read off from \eqref{eqn5.1}. We have
$$
I_{SR} = (x_1x_5x_6,x_2x_3x_4).
$$
The ideal $J$ is generated by $r_i\cdot \mathbf{x}$, $i=1,2,3,4$, where $r_i$ are the rows of $P$, and $\mathbf{x} = (x_1,x_2,\cdots,x_6)$. We have
$$
J = (x_1+x_5-2x_6,x_2-x_4+x_5-x_6,x_3-x_4+2x_5-2x_6,x_5-x_6),
$$
which gives the relations among classes
\begin{equation}\label{divrel}
D_{v_1} = D_{v_5} = D_{v_6}, \quad D_{v_2}=D_{v_3}=D_{v_4},
\end{equation}
Then we have
\begin{equation}\label{cohoXs}
H^*(X_\Sigma,\bZ)\cong \bZ[x_1,x_2\cdots,x_7]/(I_{RS}+J) \cong \bZ[x_1,x_2]/I'_{RS},
\end{equation}
where
$$
I'_{RS} = (x_1^3,x_2^3).
$$





\subsubsection{The even cohomology of $\check V$}\label{sec4.1.7}
By Baytrev mirror construction, the mirror of $V$ is the generic anti-canonical hypersurface $\check V\subset \bP_\Delta$. The anti-canonical class is $-K_{\bP_\Delta}= \sum_{i=1}^nD_{v_i} = 3D_{v_1}+3D_{v_2}$. In particular, since $-K_{\bP_\Delta}$ is ample, we know $D_{v_1}+D_{v_2}$ sits inside the K{\"a}hler cone.

First, by Lefschetz hyperplane theorem, we have
$$
i^*:H^2(\bP_\Delta,\bZ) \cong H^2(\check V,\bZ)\cong H^{1,1}(\check V,\bZ).
$$
Then $H^2(\check V,\bZ)$ is generated by $T_1:=i^*D_{v_1}, T_2:=i^*D_{v_2}$ as an abelian group. Next, since pullback preserves the K{\"a}hler cone, we have $T_1+T_2$ sitting inside the K{\"a}hler cone of $\check V$. By hard Lefschetz theorem, we have $(T_1+T_2)\cdot :H^2(\check V,\bQ)\rightarrow H^4(\check V,\bQ)$ is an isomorphism. Therefore, we have
$$
H^4(\check V,\bQ) = \bQ\braket{T_1(T_1+T_2),T_2(T_1+T_2)}.
$$
Now, we want to calculate the intersection numbers \[
\check I_{i,j} :=\int_{\check V}(T_{i}\cup T_j(T_1+T_2)),\quad i,j=1,2.
\]
By the projection formula, we have $I_{i,
j} = \int_{\bP_\Delta}3(D_{v_1}+D_{v_2})^2D_{v_i}D_{v_j} = 6-3\delta_{i,j}$. Where we have used the fact $\int_{\bP_\Delta} D_{v_1}^iD_{v_2}^j = \delta_{i,2}\delta_{j,2}$. In particular, we have $T_1T_2 = T_1^2+T_2^2$, and $T_1^2T_2 = T_1T_2^2$.


Next, since $\check V$ is smooth, the total Chern class $c(\check V)$ can be calculated by the normal sheaf sequence
\[
0\rightarrow \mathscr{T}_{\check V}\rightarrow i^*\mathscr{T}_{\bP_\Delta}\rightarrow i^*K_{\bP_\Delta}^{\otimes-1}\rightarrow 0,
\]
then
\begin{align*}
   c(\check V) & = \frac{i^*c(\bP_\Delta)}{i^*\cO(3D_{v_1}+3D_{v_2   })}= \frac{(1+T_1)^3(1+T_2)^3}{1+3(T_1+T_2)}\\
& = 1+3(T_1^2+3T_1T_2+T_2^2)-27(T_1^2T_2+T_1T_2^2) \\
& = 1+12T_1T_2-27(T_1^2T_2+T_1T_2^2)
\end{align*}
where $c(\bP_\Delta)$ is calculated by the toric Euler sequence
\[
0\rightarrow \Omega_{\bP_\Delta}^1\rightarrow \bigoplus _{i=1}^6 \mathcal{O}_{\bP_\Delta}(-D_{v_i})\rightarrow \mathrm{Pic}(\bP_{\Delta})\otimes \mathcal{O}_X\rightarrow 0.
\]
See chapter 13 of \cite{CLS11} for details. Then we have $c_2(\check V) = 3(T_1^2+3T_1T_2+T_2^2)$, and the total Todd class is $td(\check V) = 1+\frac{c_2(\check V)}{12} = 1+T_1T_2$.

Consider the following symplectic form on $K(\check V,\bQ):=K(\check V)\otimes\bQ$
\begin{align*}
   K(\check V,\bQ)\otimes K(\check V,\bQ) &\rightarrow \bQ \\
    E_1\otimes E_2&\rightarrow\chi(E_1,E_2) = \int_{\check V}ch(E_1^*)ch(E_2)td(\check V),
\end{align*}
where the last equality is given by the Hirzebruch-Riemann-Roch formula. 

Then we have a half-integral symplectic basis of $K(\check V,
bQ)$
\[
\{1 = E_1^{(0)}= [\cO_{\check V}],E_{1}^{(1)},E_{2}^{(1)},E_{2}^{(2)},E_{1}^{(2)},E_{1}^{(3)}\}
\]
where $E_{i}^{(m)}\in K(\check V,\bQ)$ supports on codimension $m$ cycle. Under the isomorphism $ch:K(\check V,\bQ)\rightarrow H^{even}(\check V,\bQ)$, their total Chern characteristics are
\[
\{1,(T_1-\sum_{l}\frac 12 C_{1l}K_l)td^{-1}_{\hat X_0},(T_2-\sum_{l}\frac 12 C_{2l}K_l)td^{-1}_{\hat X_0},K_2,K_1,V\} 
\]
where $K_1 = \frac{T_2^2}{3}$, $K_2 = \frac{T_1^2}{3}$ satisfies $\int_{\check 
V}T_iK_j = \delta_{i,j}$; $V = -\frac{T_1^2T_2+T_1T_2^2}{6}$, satisfies $\int_{\check V}V = -1$. The $C_{i,j}$ are some integers undetermined integers.

\subsubsection{Hosono's $w$-function}
The principal period can be read off from \eqref{susfan5.2}
\[
w = \sum_{n_1,n_2\geq0}\frac{\Gamma(3(n_1+n_2)+1)}{\Gamma(n_1+1)^3\Gamma(n_2+1)^3}z_1^{n_1}z_2^{n_2}.
\]

The Hosono's $w$-function is a $H^{even}(\check V,\bC)$-valued function on $\bar B$, that is closed related to the Givental's $I$-function, which in our case it is
\begin{equation}\label{wbasexpan}
\begin{split}
    w  = & w_0\cdot ch(E_1^{(0)})+ w_{1}^{(1)}\cdot ch(E_1^{(1)})+ w_1^{(2)}\cdot ch(E_1^{(2)})+ w_2^{(2)}ch(E_{2}^{(2)}) \\
    & + w_1^{(2)}\cdot ch(E_{1}^{(2)}) +w_3 \cdot ch(E_1^{(3)})\\
    = & w_0 + w_1^{(1)}T_1+w_2^{(1)}T_2+(w_1^{(2)}-\frac{C_{11}}{2}w_1^{(1)}-\frac{C_{21}}{2}w_2^{(1)})K_1\\
    & + (w_2^{(2)}- \frac{C_{12}}{2}w_1^{(1)}-\frac{C_{22}}{2}w_2^{(1)})K_2 + (3w_{1}^{(1)}+3w_{1}^{(1)}+w_3)V.
\end{split}
\end{equation}
Then we have
\begin{align*}
    &w_0 = w|_{T_i=0}, \quad w_1^{(1)}= \partial_{T_1}w|_{T_i=0},  \quad w_2^{(1)} = \partial_{T_2}w|_{T_i=0}, \\
    & w_2^{(2)} = \frac32 \partial_{T_1}^2w|_{T_i=0}+3\partial_{T_1}\partial_{T_2}w|_{T_i=0}+\frac{C_{12}}{2}\partial_{T_1}w|_{T_i=0}+\frac{C_{22}}{2}\partial_{T_2}w|_{T_i=0},\\
    & w_1^{(2)} = \frac32 \partial_{T_2}^2w|_{T_i=0}+3\partial_{T_1}\partial_{T_2}w|_{T_i=0}+\frac{C_{11}}{2}\partial_{T_1}w|_{T_i=0}+\frac{C_{21}}{2}\partial_{T_2}w|_{T_i=0},\\
    & w_3 = -\frac{3}{2}(\partial_{T_1}^2\partial_{T_2}w|_{T_i=0}+\partial_{T_1}\partial^2_{T_2}w|_{T_i=0}) - 3\partial_{T_1}w|_{T_i=0}-3\partial_{T_2}w|_{T_i=0}.
\end{align*}

The monodromy of these functions is given by
$$
\left[
\begin{array}{l}
     w_0\\
     w_1^{(1)}\\
     w_2^{(1)}\\
     w_2^{(2)}\\
     w_1^{(2)}\\
     w^{(3)}\\
\end{array}
\right] \xrightarrow{z_1\rightarrow e^{2\pi i}z_1} \left[
\begin{array}{ccccccc}
     1 & 0 & 0 & 0 & 0 & 0 \\
     1 & 1 & 0 & 0 & 0 & 0 \\
     0 & 0 & 1 & 0 & 0 & 0 \\
     \frac{C_{12}+3}{2} & 3 & 3 & 1 & 0 & 0\\
     \frac{C_{11}}{2} & 0 & 3  & 0 & 1 & 0\\
     -3 & \frac{C_{11}}{2}  & \frac{C_{21}-3}{2} & 0 & -1 & 1
\end{array}
\right]\cdot
\left[
\begin{array}{l}
     w_0\\
     w_1^{(1)}\\
     w_2^{(1)}\\
     w^{(3)}\\
     w_1^{(2)}\\
     w_2^{(2)}\\
\end{array}
\right],
$$
and
$$
\left[
\begin{array}{l}
     w_0\\
     w_1^{(1)}\\
     w_2^{(1)}\\
     w^{(3)}\\
     w_1^{(2)}\\
     w_2^{(2)}\\
\end{array}
\right] \xrightarrow{z_1\rightarrow e^{2\pi i}z_1} \left[
\begin{array}{ccccccc}
     1 & 0 & 0 & 0 & 0 & 0 \\
     0 & 1 & 0 & 0 & 0 & 0 \\
     1 & 0 & 1 & 0 & 0 & 0 \\
     \frac{C_{22}}{2} & 3 & 0 & 1 & 0 & 0\\ 
     \frac{C_{21}+3}{2} & 3 & 3 & 0 & 1 & 0\\
     -3 & \frac{C_{12}-3}{2} & \frac{C_{22}}{2} & -1 & 0 & 1
\end{array}
\right]\cdot
\left[
\begin{array}{l}
     w_0\\
     w_1^{(1)}\\
     w_2^{(1)}\\
     w^{(3)}\\
     w_1^{(2)}\\
     w_2^{(2)}\\
\end{array}
\right],
$$
Denote these two matrices as $S_1,S_2$. They are symplectic with respect to the standard symplectic
\begin{equation}\label{strdsympl}
Q^{st}:=\left[\begin{array}{cccccc}0 & 0 & 0 & 0 & 0 & -1 \\0 & 0 & 0 & 0 & -1 & 0 \\0 & 0 & 0 & -1 & 0 & 0 \\0 & 0 & 1 & 0 & 0 & 0 \\0 & 1 & 0 & 0 & 0 & 0 \\1 & 0 & 0 & 0 & 0 & 0\end{array}\right],
\end{equation}
we have $C_{12} = C_{21}$. As can be checked easily, these two monodromies are simply
\[
v\rightarrow S_i\cdot v = ch(\cO(-T_i))\cup v = e^{-T_i}\cup v,\quad \forall v\in H^{even}(\check V,\bQ).
\]



\subsection{$V_{(2,38)}$}
The toric data for this case is given by
\begin{equation}
\begin{array}{c|ccccccc}
\Xi&  v_1 &  v_2 &  v_3 &  v_4 &v_5 \\
\hline
 r_1 & 1 & 0 & 0 & 1 & -4 \\
 r_2 & 0 & 1 & 0 & 2 & -5 \\
 r_3 & 0 & 0 & 1 & 1 & -2 \\
 r_4 & 0 & 0 & 0 & 3 & -3 \\
\hline
 w_1 & 1 & 1 & 0 & 0 & 0 \\
 w_2 & 0 & 0 & 1 & 1 & 1 
\end{array}.
\end{equation}
Then, we have $X_\Sigma$ is a quotient of $\bP[3,3,1,1,1]$ by $\bZ/3\bZ$, and the Baytrev mirror of $X_\Sigma$ is $\bP_{\Delta^\circ}$. However, since $X_\Sigma$ has more than terminal singularity, we need to conduct a toric resolution by adding an additional column $(-1,-1,0,0)^t$. We will denote the new fan still as $\Sigma$. Then the suspended toric data is
\begin{equation}
\begin{array}{c|ccccccc}
\bar\Xi& \bar v_1 & \bar v_2 & \bar v_3 &\bar  v_4 &\bar  v_5 &\bar  v_6 &\bar  v_7\\
\hline
\bar r_1 & 1 & 0 & 0 & 1 & -4 & -1 & 0\\
\bar r_2 & 0 & 1 & 0 & 2 & -5 & -1 & 0\\
\bar r_3 & 0 & 0 & 1 & 1 & -2 & 0 & 0\\
\bar r_4 & 0 & 0 & 0 & 3 & -3 & 0 & 0\\
\bar r_5 & 1 & 1 & 1 & 1 & 1 & 1 & 1\\
\hline
\bar w_1 & 1 & 1 & 0 & 0 & 0 & 1 & -3\\
\bar w_2 & 0 & 0 & 1 & 1 & 1 & -3 & 0
\end{array}.
\end{equation}


\subsubsection{Moduli spaces}
Since $\Delta^\circ_{345}$ has an integral interior point $v_7$, in order to show $\cM_{\mathrm{poly}}=\cM$, we need to show the dual face of $\Delta^\circ_{345}$ has no integral interior point. A direct calculation gives that the dual face is the interval between $v^\circ_1,v^\circ_2\in M$, with $v^\circ_1 = (-1,2,-1,-1)$, and $v^\circ_2 = (2,-1,-1,0)$. Thus, we have $\cM_{\mathrm{poly}}=\cM$. It is also clear from the muti-degrees that $\tAut_r(\bP_{\Delta^\circ})$ is trivial.

The fan symmetry of $\tAut(\Sigma)$ the group $S_3$ which is generated by $(12)(34)$ and $(345)$.
 A generic point in $\bP(L(\Delta^\circ\cap N))$ is given by
\[
f = \lambda_1 t_1+\lambda_2t_2+\lambda_3t_3+\lambda_4 t_1t_2^2t_3t_4^3+\lambda_5t_1^{-4}t_2^{-5}t_3^{-2}t_4^{-3}+\lambda_6t_1^{-1}t_2^{-1}+\lambda_7,
\]
One can easily check both $(12)(34)$ and $(345)$ can be realized as a $T$ action, thus $\tAut(\Sigma)$ acts on $\cM_{\mathrm{simp}}$ trivially. Therefore, we have $\cM_{\mathrm{simp}}  = \cM$.

The secondary fan $\Sigma^s$ is
\begin{equation}
\frac{A^s}{B^s} = \begin{array}{c|cccc}
\Xi^s&v_1^s & v_2^s & v_3^s & v_4^s \\
\hline
r_1^s & 1 & 0 & 1 & -1\\
r_2^s & 0 & 1 & -3 & 0\\
\hline
w_1^s & 1 & 0 & 0 & 1 \\
w_2^s & 0 & 3 & 1 & 1 \\
\end{array}.
\end{equation}
Then $\overline{\cM}_{\mathrm{simp}} \cong \bP_{\Delta^s}$ is a smooth toric varies. More concretely, we have $\bP_{\Delta^s}\cong \mathrm{Proj}_{B^s}\bC[Z_1,Z_2,Z_3,Z_4]$, with $Z_i$ has multi-degree $(w_{1,i}^s,w_{2,i}^s)$. Then the canonical affine coordinates are
\[
z_1 = \frac{\lambda_1\lambda_2\lambda_6}{\lambda_7^3} = \frac{Z_1Z_3}{Z_4},\quad z_2 =  \frac{\lambda_3\lambda_4\lambda_5}{\lambda_6^3} = \frac{Z_2}{Z_3^3}.
\]

\subsubsection{Picard-Fuchs equations and discriminant locus}
\begin{align*}
    & P_1 = \delta_1(\delta_1-3\delta_2) +3z_1(3\delta_1+1)(3\delta_1+2)\\
    & P_2 = \delta_2^3-z_2(\delta_1-3\delta_2)(\delta_1-3\delta_2-1)(\delta_1-3\delta_2-2)
\end{align*}
For simplicity, we rescale the local coordinates as $z_{1,2}':=3^3\cdot z_{1,2}$, and rename $z_{1,2}'$ as the new $z_{1,2}$. The Picard-Fuchs operators become
\begin{align*}
    & P_1 = \delta_1(\delta_1-3\delta_2) +z_1(\delta_1+\frac13)(\delta_1+\frac23)\\
    & P_2 = \delta_2^3-z_2(\frac13\delta_1-\delta_2)(\frac13\delta_1-\delta_2-\frac13)(\frac13\delta_1-\delta_2-\frac23)
\end{align*}
The singular locus contains inside
\[
D_A \cup  D_1 \cup D_{v_1^s}\cup D_{v_2^s}\cup D_{v_3^s}\cup D_{v_4^s}
\]
where $D_A = (1+z_1)^3+z_1^3z_2$, $D_1 = 1+z_2$. In this affine chart, we have $D_{v_1^s}$ intersects $D_{v_2^s}$ transversely at origin; 
The $D_A$ intersects $D_{v_2^s} = \bV(z_2)$ at $(z_1,z_2) = (-1,0)$ with 3-tangency and thus requires to be blown up three times, with the exceptional divisors denoted as $E_1,E_2,E_3$;
The $D_1$ intersects $D_{v_1^s}$ transversally at one point $(z_1,z_2) = (0,-1)$. 
Now, there are intersections outside this affine chart. Now, switch back to the original $z_1,z_2$ coordinates before the rescaling and let
\[
z_1' = \frac{Z_1Z_2^{\frac13}}{Z_4},\quad z_2' = \frac{Z_3}{Z_2^{\frac13}},
\]
we have
\[
z_1 = z_1'z_2',\quad z_2 = z_2'^{-3},
\]
Since the coordinates change is étale away from the boundaries, the Picard-Fuchs ideal becomes
\[
\begin{split}
 & P_1 = \delta_1'\delta_2' +3z_1'z_2'(3\delta_1'+1)(3\delta_1'+2)\\
 & P_2 = z_2'^3(\delta_1'-\delta_2')^3-\delta_2'(\delta_2'-1)(\delta_2'-2)
 \end{split}
\]
Similar, by a rescale $z_{1}'':=3^4\cdot z_{1}'$, $z_{2}'':=3^{-1}\cdot z_{2}'$, and rename $z_{1,2}''$ as the new $z_{1,2}'$, then $D_A = (1+z_1'z_2')^3+z_1'^3$, $D_1 = 1+z_2^{-3}$, and
\[
\begin{split}
 & P_1 = \delta_1'\delta_2' +z_1'z_2'(\delta_1'+\frac13)(\delta_1'+\frac23)\\
 & P_2 = 27z_2'^3(\delta_1'-\delta_2')^3-\delta_2'(\delta_2'-1)(\delta_2'-2),
 \end{split}
\]
In this affine chart we have additionally two cones that correspond to $D_{v_2^s}$ intersects $D_{v_3^s}$ transversely at origin, and $D_A$ intersects $D_{v_3^s}$ transversely at $(-1,0)$. The last affine chart that we would want to consider is 
\[
z_1'' = z_1^{-1},\quad z_2'' = z_2,
\]
where $z_i$ are the original $z_i$ before rescale. Then the Picard-Fuchs ideal is
\begin{align*}
    & P_1 = z_1\delta_1(\delta_1+3\delta_2) +3(3\delta_1-1)(3\delta_1-2)\\
    & P_2 = \delta_2^3+z_2(\delta_1+3\delta_2)(\delta_1+3\delta_2+1)(\delta_1+3\delta_2+2),
\end{align*}
Similar, by a rescale $z_{1}''':=3^{-3}\cdot z_{1}'$, $z_{2}'':=3^{3}\cdot z_{2}'$, and rename $z_{1,2}''$ as the new $z_{1,2}'$, then $D_A = (1+z_1)^3+z_2$, $D_1 = 1+z_2$, and
\begin{align*}
    & P_1 = z_1\delta_1(\delta_1+3\delta_2) +(\delta_1-\frac13)(\delta_1-\frac23)\\
    & P_2 = \delta_2^3+z_2(\frac13\delta_1+\delta_2)(\frac13\delta_1+\delta_2+\frac13)(\frac13\delta_1+\delta_2+\frac23),
\end{align*}
This time, $D_A$ intersects $D_1$ and $D_{v_4^s}$ at a triple intersection point $(0,-1)$. Thus we need to blow up this point once, and the exceptional divisor is denoted as $E_0$. Since $D_{v_4^s}$ has finite monodromy, the only new possible two-dimension cones in this chart are those associated to $D_A\cap E_0$ and $D_1\cap E_0$.


\begin{remark}
    All the rescales in this section can be done simultaneously in the homogeneous coordinates $Z_i$ by rescaling $Z_1,Z_2$ by a $3^3$ factor.
\end{remark}

\subsubsection{Nilpotent cones}
 we can take the global multi-valued frame 
\[
w = (\Omega,\delta_1\Omega,\delta_2\Omega,\delta_1\delta_2\Omega,\delta_2^2\Omega,\delta_2^2\delta_1\Omega).
\]
\[
N_1 =\left[
\begin{array}{cccccc}\label{eqn:monomatricesv238}
    0 & 0  & 0 & 0 & 0 & 0  \\ 
    1 & 0  & 0 & 0 & 0 & 0 \\ 
    0 & 0 &  0&  0&  0&  0\\ 
    0 & 3 & 1 & 0 & 0 & 0  \\ 
    0 & 0 & 0 & 0 & 0 & 0  \\ 
    0 & 0 & 0 & 3 & 1 &  0 \\ 
\end{array}
\right],\quad N_2 =\left[
\begin{array}{cccccc}
    0 & 0  & 0 & 0 & 0 & 0  \\ 
    0 & 0  & 0 & 0 & 0 & 0 \\ 
    1 & 0 &  0&  0&  0&  0\\ 
    0 & 1 & 0 & 0 & 0 & 0  \\ 
    0 & 0 & 1 & 0 & 0 & 0  \\ 
    0 & 0 & 0 & 1 & 0 &  0 \\ 
\end{array}
\right],
\]

\begin{align}
 \label{cone21}    \mathrm{Cone}(D_{v_1^s},D_{v_2^s}) & = \braket{IV_1|IV_2|III_0}\\
 \label{cone22}    \mathrm{Cone}(D_{v_2^s},E_3) & = \braket{III_0|III_0(IV_2)|III_0}\\
 \label{cone23}    \mathrm{Cone}(E_1,E_2) & = \braket{III_0|III_0(IV_2)|III_0}\\
 \label{cone24}    \mathrm{Cone}(E_2,E_3) & = \braket{III_0|III_0(IV_2)|III_0}\\
 \label{cone25}    \mathrm{Cone}(D_A,E_3) & = \braket{I_1|III_0(IV_2)|III_0}\\
    \label{cone26}    \mathrm{Cone}(D_{v_1^s},D_1) & = \braket{IV_1|IV_2|I_1}\\
    \label{cone27}    \mathrm{Cone}(D_{v_2^s},D_{v_3^s}) & = \braket{III_0|III_0(IV_2)|I_1}\\
    \label{cone28}    \mathrm{Cone}(D_{v_3^s},D_A) & = \braket{I_1|I_2(I_1)|I_1}\\
    \label{cone29}    \mathrm{Cone}(D_{v_1^s},D_{v_3^s}) & = \braket{IV_1|IV_2|I_1}\\
        \label{cone210}    \mathrm{Cone}(D_{A},E_0) & = \braket{I_1|III_0(IV_2)|III_0}\\
        \label{cone211}    \mathrm{Cone}(D_{1},E_0) & = \braket{I_1|III_0(IV_2)|III_0}
\end{align}

\subsubsection{Even cohomology of $\check V$ and monodromy}
By the same calculation in Section \ref{sec4.1.7}, we have
$$
H^*(\bP_\Delta,\bZ) \cong \bZ[x_1,x_2\cdots,x_6]/(I_{RS}+J).
$$
with
$$
I_{SR} = (x_1x_6,x_2x_6,x_3x_4x_5)
$$
and
\[
J = (x_1+x_4-4x_5-x_6,x_2+2x_4-5x_5-x_6,x_3+x_4-2x_5,3x_4-3x_5).
\]
Then we have $D_{v_3} = D_{v_4} = D_{v_5}$, $D_{v_1} = D_{v_2}$, $D_{v_6} = D_{v_1}-3D_{v_3}$, and
\[
H^*(\bP_\Delta,\bZ)\cong \bZ[x_1,x_3]/(x_1^2-3x_1x_3,x_3^3),
\]
Similarly, we have $K_{\bP_\Delta} = -3D_{v_1}$ is an ample divisor. Take $T_1:=i^*D_{v_1}, T_2:=i^*D_{v_3}$, then we have $H^{even}(\check V,\bZ)$ is generated by $T_1,T_2$ that satisfies the relation

\subsection{$V_{(2,86)}$, the mirror octic}
This is the smooth Calabi-Yau 3-fold mirror to the 
the smooth anti-canonical hypersurface in $\bP[1,1,2,2,2]$. This family is very similar to the case of $V_{(2,38)}$. The mirror symmetry of this family is studied in detail in \cite{COFK94,CK99}. The first author calculated the nilpotent fan for the family in \cite{Chen23}. The two-dimensional nilpotent cones are 
\begin{align*}
    & \sigma_{12} = 
    \braket{IV_2|IV_2|II_1},
    && \sigma_{13} = \braket{IV_2|IV_2|I_1},\\
    &\sigma_{34} = 
    \braket{I_1|I_2|I_1},
    && \sigma_{45} =
    \braket{I_1|II_1|II_0}, \\
    & \sigma_{52} =
    \braket{II_0|II_1|II_1},
    && \sigma_{63} = 
    \braket{I_1|I_2|I_1}, \\
    & \sigma_{67} =
    \braket{I_1|I_2|I_1}.
\end{align*}
The nilpotent operators $N_1,N_2$ corresponding to the cone $\sigma_{12}$ is given by 





==> 6star-Copy.tex <==

% ---------------------------------------
\section{Examples: Calabi-Yau 3-folds in toric variety}

In this section, we will calculate the generic degree of the period map of type (1,2,2,1) that arises from the tautological family of Calabi-Yau hypersurfaces inside the toric variety.

The subsections will be named after the Hodge type of the Calabi-Yau 3-folds, namely in subsection $V_{(a,b)}$, we will study 

% ---------------------------------------

\subsection{$V_{(2,29)}$}
We study the smooth Calabi-Yau 3-folds $V$ with Hodge numbers $(h^{2,1},h^{1,1}) = (2,29)$, which is the anti-canonical hypersurface of the toric variety $X_{\Sigma^\circ}\cong \bP_{\Delta^\circ}$. The toric data for $\Delta^\circ$ and $\Sigma$ is
\begin{equation}\label{eqn5.1}
\frac{A}{B}=
\begin{array}{c|cccccc}
\Xi&v_1 & v_2 & v_3 & v_4 & v_5 & v_6\\
\hline
r_1 & 1 & 0 & 0 & 0 & 1 & -2\\
r_2 & 0 & 1 & 0 & -1 & 1 & -1\\
r_3 & 0 & 0 & 1 & -1 & 2 & -2\\
r_4 & 0 & 0 & 0 & 0 & 3 & -3\\
\hline
w_1 & 1 & 0 & 0 & 0 & 1 & 1\\
w_2 & 0 & 1 & 1 & 1 & 0 & 0
\end{array}.
\end{equation}
The polytope $\Delta^\circ$ can be visualized as follows: $\Xi$ is naturally divided into two sets $\{v_1,v_5,v_6\}$ and $\{v_2,v_3,v_4\}$ where the points in both sets lie in the same plane, the 9 facets of $\Delta$ then come from choosing two points from each set.
After suspension, the toric data becomes
\begin{equation}\label{susfan5.2}
\frac{\bar A}{\bar B}=
\begin{array}{c|ccccccc}
\bar\Xi& \bar v_1 & \bar v_2 & \bar v_3 &\bar  v_4 &\bar  v_5 &\bar  v_6 &\bar  v_7\\
\hline
\bar r_1 & 1 & 0 & 0 & 0 & 1 & -2 & 0\\
\bar r_2 & 0 & 1 & 0 & -1 & 1 & -1 & 0\\
\bar r_3 & 0 & 0 & 1 & -1 & 2 & -2 & 0\\
\bar r_4 & 0 & 0 & 0 & 0 & 3 & -3 & 0\\
\bar r_5 & 1 & 1 & 1 & 1 & 1 & 1 & 1\\
\hline
\bar w_1 & 1 & 0 & 0 & 0 & 1 & 1 & -3\\
\bar w_2 & 0 & 1 & 1 & 1 & 0 & 0 & -3
\end{array}.
\end{equation}


\subsubsection{Moduli spaces}
The toric data shows that $(\Delta^\circ \cap N)_0 = \Delta^\circ \cap N$, i.e., there is no integral point lies in the interior of codimension 2 face. Therefore, we have $\cM = \cM_{\mathrm{poly}}$.

The generic degree of the map $\phi:\cM_{\mathrm{poly}} \rightarrow  \cM_{\mathrm{simp}}$
is $|\tAut(\Delta^\circ)/\tAut^{t}(\Delta^\circ)|$, where $\tAut^{t}(\Delta^\circ)$ is the normal subgroup of $\tAut(\Delta^\circ)$ that acts trivially on $\cM_{\mathrm{poly}}$. 

Denote $\tAut(\Xi)$ as the subgroup of $\tAut(N)$ that permutes $\Xi$, then a direct calculation shows $\tAut(\Xi) = C_2\times C_3\rtimes S_3$, which acts on $\Xi$ as follows: the $C_2$ factor determines whether the permutation is even or odd, the set $\{v_2,v_3,v_4\}$ is sent to $\{v_2,v_3,v_4\}$ or $\{v_1,v_5,v_6\}$ respectively for the two cases. Then the $S_3$ factor determines the image of $v_2,v_3,v_4$ under the automorphism, and since the parity of the permutation is already determined, there are only $C_3$ choices for the image of $v_1,v_5,v_6$. From this description, it is also clear that every element in $\tAut(\Xi)$ permits the facets of $\Delta^\circ$, thus we have
$\tAut(\Delta^\circ) = \tAut(\Xi)$. As a subgroup of $S_6$ which acts on $\Xi$ by permutation, we have $\tAut(\Delta^\circ)$ is generated by the permutations $a:= (234),b:=(34)(56),c:=(12)(35)(46)$. 






A generic point in $\bP(L(\Delta^\circ\cap N))$ is given by
\[
f = \lambda_1 t_1+\lambda_2t_2+\lambda_3t_3+\lambda_4 t^{-1}_2t_3^{-1}+\lambda_5t_1t_2t_3^2t_4^3+\lambda_6t_1^{-2}t_2^{-1}t_3^{-2}t_4^{-3}+\lambda_7,
\]
Then we have
\[
a\cdot f = \lambda_1 t_1+\lambda_3t_2+\lambda_4t_3+\lambda_2 t^{-1}_2t_3^{-1}+\lambda_5t_1t_2t_3^2t_4^3+\lambda_6t_1^{-2}t_2^{-1}t_3^{-2}t_4^{-3}+\lambda_7,
\]
which can be realized as a $T$-action 
\[
(t_1,t_2,t_3,t_4)\rightarrow (t_1,\lambda_2^{-1}\lambda_3t_2,\lambda_3^{-1}\lambda_4t_3,\lambda_2^{1/3}\lambda_3^{1/3}\lambda^{-2/3}_4t_4),
\]
similarly, $b$ can be realized as
\[
(t_1,t_2,t_3,t_4)\rightarrow (t_1,t_2,\lambda_3^{-1}\lambda_4t_3,\lambda_3^{2/3}\lambda^{-2/3}_4\lambda_5^{-1/3}\lambda_6^{1/3}t_4).
\]
However, $c$ can not be realized as a $T$-action, therefore, we have $\tAut^t(\Delta^\circ) = C_3\rtimes S_3$, and the generic degree of $\phi$ is
\[
\deg_g(\phi)=|\tAut(\Delta^\circ)/\tAut^t(\Delta^\circ)|=2.
\]

The toric data for the secondary fan $\Sigma^s$ is
\begin{equation}
\frac{A^s}{B^s}=
\begin{array}{c|ccc}
\Xi^s&v_1^s & v_2^s & v_3^s \\
\hline
r_1^s & 1 & 0 & -1 \\
r_2^s & 0 & 1 & -1 \\
\hline
w_1^s & 1 & 1 & 1 \\
\end{array}.
\end{equation}
Therefore, $\overline{\cM}_{\mathrm{simp}} = X_{\Sigma^s} \cong \bP^2 = \mathrm{Proj}\bC[Z_1,Z_2,Z_3]$.








\subsubsection{Picard-Fuchs system}
The GKZ ideal is generated by the Euler vectors $Z_i = \sum_{j=1}\bar v_{i,j}\delta_j - \beta_i$, $i=1,\dots,5$, $\beta_i = \delta_{i,5}$ and the toric ideal

The canonical affine chart is $\tSpec[z_1,z_2]$, with
\[
z_1 = \frac{\lambda_1\lambda_5\lambda_6}{\lambda_7^2},\quad z_2 = \frac{\lambda_2\lambda_3\lambda_4}{\lambda_7^2},
\]
then $D_{v_1^s} = \bV(z_1)$, $D_{v_{1^s}} = \bV(z_2)$. In the projective coordinates, this is the chart with $Z_3\neq 0$, and $z_i = \frac{X_i}{X_3}, i=1,2$.

The Picard-Fuchs ideal on $\cM$ is generated by the two differential operators
\begin{align*}
    & P_1:= \delta_1^3+z_1(3\delta_1+3\delta_2+1)(3\delta_1+3\delta_2+2)(3\delta_1+3\delta_2+3),\\
    & P_2:= (\delta_1^2-\delta_1\delta_2+\delta_2^2)+3(z_1+z_2)(3\delta_1+3\delta_2+1)(3\delta_1+3\delta_2+2).
\end{align*}
For simplicity, we rescale the local coordinates as $z_{1,2}':=3^3\cdot z_{1,2}$, and rename $z_{1,2}'$ as the new $z_{1,2}$. The Picard-Fuchs operators then become
\begin{equation}\label{eqp1p2}
\begin{aligned}
    & P_1:= \delta_1^3+z_1(\delta_1+\delta_2+\frac13)(\delta_1+\delta_2+\frac23)(\delta_1+\delta_2+1),\\
    & P_2:= (\delta_1^2-\delta_1\delta_2+\delta_2^2)+(z_1+z_2)(\delta_1+\delta_2+\frac13)(\delta_1+\delta_2+\frac23).
\end{aligned}
\end{equation}
The Picard-Fuchs ideal sheaf is denoted as $I$, which in the canonical affine affine chart is generated by $P_1$ and $P_2$. The associated $\cD$-module is clearly $\bZ/2\bZ$-equivariant under $z_1\leftrightarrow z_2$, $\partial_1\leftrightarrow \partial_2$.


\subsubsection{Discriminant locus}
The principal $A$-determinant $E_A$ is irreducible, and is thus equals to the $A$-discriminant $D_A$
\begin{align*}
D_A = & z_1^3 + 3z_1^2z_2 + 3z_1^2 + 3z_1z_2^2 - 21z_1z_2 + 3z_1 + z_2^3 + 3z_2^2 + 3z_2 + 1\\
 = & (z_1+z_2+1)^3-27z_1z_2
\end{align*}
so the discriminant locus is contained inside
\[
Disc= D_A\cup (\bar B\setminus B) = D_A\cup D_{v_1^s}\cup D_{v_2^s}\cup D_{v_3^s}.
\]

In the canonical affine chart $D_A$ intersect $D_{v_1^s}$ at $(-1,0)$ with 3-tangency, and by the $\bZ/2\bZ$ symmetry, $D_A$ intersect $D_{v_2^s}$ at $(0,-1)$ with 3-tangency.

In order to make $Disc$ only have normal crossing singularities, we need to blow-up these tangencies 3 times each. Since we will only be interested in the local monodromy, we only need to study the geometry at $z_1 = 0, z_2 = -1$. Denote the exceptional divisors of the three blow-ups as $E_1,E_2,E_3$, then we want to find 4 Picard-Fuchs ideals corresponding to the normal crossings 
\[
D_{v_1}\cap E_3, \quad E_1\cap E_2,\quad E_2\cap E_3\quad D_A\cap E_3,
\]
First, we make a change of coordinate of \eqref{eqp1p2} by $z_1 \rightarrow z_1$, $z_2\rightarrow z_2-1$. Then the local affine coordinates systems for each of the normal crossing is given by
\begin{equation*}
 \begin{aligned}
     & (s,t) = \left(\frac{z_1}{z_2^3},z_2\right),\quad && (s,t)= \left(\frac{z_2^2}{z_1},\frac{z_1}{z_2}\right),\\
     & (s,t)= \left(\frac{z_2^3}{z_1},\frac{z_1}{z_2^2}\right), \quad && (s,t) = \left(\frac{z_1}{z_2^3}-\frac{1}{27},z_2\right)
 \end{aligned}   
\end{equation*}
With $s=0$ gives the left divisor and $t=0$ gives the right divisor.

To see this, the local geometry of the first blow-up is given by 
\[
\mathrm{Proj}_{(0,0,1,1)}(\bC[z_1,z_2,X,Y]/(z_1Y-z_2X)),
\]
Since the 

Then the Picard-Fuchs ideal can be written locally with respect to this change of coordinates.

One useful identity is
\[
\partial_i^n = \frac{1}{z_i^n}\prod_{k=0}^{n-1}(\delta_i-k)
\]
The initial ideals are generated by
\begin{equation}
\begin{aligned}
    & P_1^{(1)}:= 
    (\delta_1+3\delta_2)^3, &&P_2^{(1)}:= 10\delta_2^2 + 3\delta_1\delta_2;\\
    & P_1^{(1)}:=(\delta_1+\delta_2)(\delta_1+\delta_2-1)(\delta_1+\delta_2-2), && P_2^{(2)}:=5\delta_1^2 + 7\delta_1\delta_2 + 2\delta_2^2;\\
    & P_1^{(3)}:= (5\delta_1+2\delta_2)^3, && P_2^{(3)}=16\delta_1^2+23\delta_1\delta_2+7\delta_2^2+\delta_1+\delta_2;\\
    & P_1^{(4)}:= \delta_1^3, && P_2^{(3)}=\delta_1\delta_2;\\
\end{aligned}
\end{equation}


\begin{equation}
\begin{aligned}
    & P_1^{(1)}:= 
    (\delta_1+3\delta_2)^3, &&P_2^{(1)}:= \delta_2(27\delta_1+90\delta_2-8);\\
    & P_1^{(1)}:=(\delta_1+\delta_2)(\delta_1+\delta_2-1)(\delta_1+\delta_2-2), && P_2^{(2)}:=5\delta_1^2 + 7\delta_1\delta_2 + 2\delta_2^2;\\
    & P_1^{(3)}:= (5\delta_1+2\delta_2)^3, && P_2^{(3)}=16\delta_1^2+23\delta_1\delta_2+7\delta_2^2+\delta_1+\delta_2;\\
    & P_1^{(4)}:= \delta_1^3, && P_2^{(3)}=\delta_1\delta_2;\\
\end{aligned}
\end{equation}


\subsubsection{Gauss-Manin connection}
Take $w = (1,\delta_1,\delta_2,\delta_1\delta_2,\delta_1^2,\delta_1^2\delta_2).$
\[
\begin{split}
&\nabla_{\delta_1} w =
w \left[
\begin{array}{rrrrrr}
     0 & 0 & 0 & 0 & z_1h^1_{15} & z_1h^1_{16} \\
     1 & 0 & 0 & 0 & z_1h^1_{25} & z_1h^1_{26}  \\
     0 & 0 & 0 & 0 & z_1h^1_{35} & z_1h^1_{36} \\
     0 & 0 & 1 & 0 & z_1h^1_{45} & z_1h^1_{46} \\
     0 & 1 & 0 & 0 & z_1h^1_{55} & z_1h^1_{56} \\
     0 & 0 & 0 & 1 & z_1h^1_{65} & z_1h^1_{66}
\end{array}
\right],\\
&\nabla_{\delta_2} w =
w \left[
\begin{array}{rrrrrr}
     0 & 0 & z_2h^2_{1,3} & z_2h^2_{1,4} & 0 & z_2h^2_{1,6}  \\
     0 & 0 & z_2h^2_{2,3} & z_2h^2_{2,4} & 0  & z_2h^2_{2,6} \\
     1 & 0 & z_2h^2_{3,3} & z_2h^2_{3,4} & 0 & z_2h^2_{3,6}  \\
     0 & 1 & 1+z_2h^2_{4,3} & z_2h^2_{4,4} & 0  & z_2h^2_{4,6} \\
     0 & 0 & -1 & z_2h^2_{4,4}& 0  & z_2h^2_{5,6} \\
     0 & 0 & 0 & 1+z_2h^2_{5,4} & 1 & z_2h^2_{6,6}
\end{array}
\right],
\end{split}
\]
 where $h^{i}_{lm}(z_1,z_2)$ are rational functions that is holomorphic at $z_1=z_2=0$. 


\subsubsection{Monodromy and nilpotent cones}
If we choose the base point $b\in\cM_{\mathrm{simp}}$ close to $z_1=z_2=0$, or more precisely, consider
\[
N_1 =\left[
\begin{array}{cccccc}
    0 & 0  & 0 & 0 & 0 & 0  \\ 
    1 & 0  & 0 & 0 & 0 & 0 \\ 
    0 & 0 &  0&  0&  0&  0\\ 
    0 & 0 & 1 & 0 & 0 & 0  \\ 
    0 & 1 & 0 & 0 & 0 & 0  \\ 
    0 & 0 & 0 & 1 & 0 &  0 \\ 
\end{array}
\right],\quad N_2 =\left[
\begin{array}{cccccc}
    0 & 0  & 0 & 0 & 0 & 0  \\ 
    0 & 0  & 0 & 0 & 0 & 0 \\ 
    1 & 0 &  0&  0&  0&  0\\ 
    0 & 1 & 1 & 0 & 0 & 0  \\ 
    0 & 0 & -1 & 0 & 0 & 0  \\ 
    0 & 0 & 0 & 1 & 1 &  0 \\ 
\end{array}
\right],
\]


When one parallel transports the basis $w$ around a loop $l\subset \cM_{\mathrm{simp}}$, the monodromy matrix represented in the basis is defined by $w\rightarrow w\cdot T_l$. 


Similarly, at the other local charts, we take the local basis to be
\begin{align*}
    &w^{(1)} = (1,\delta_1,\delta_2,\delta_1\delta_2,\delta_1^2,\delta_1^2\delta_2)\\
    & w^{(2)} = (1,\delta_1,\delta_2,\delta_1\delta_2,\delta_1^2,\delta_1^2\delta_2)\\
    &w^{(3)} = (1,\delta_1,\delta_2,\delta_1\delta_2,\delta_1^2,\delta_1^2\delta_2)\\
    &w^{(4)} = (1,\delta_1,\delta_2,\delta_1^2,\delta_2^2,\delta_2^3)
\end{align*}

\begin{align*}
    &w^{(1)} = (1,\delta_1,\delta_2,\delta_1\delta_2,\delta_1^2,\delta_1^2\delta_2)\\
    & w^{(2)} = (1,\delta_1,\delta_2,\delta_1\delta_2,\delta_1^2,\delta_1^2\delta_2)\\
    &w^{(3)} = (1,\delta_1,\delta_2,\delta_1\delta_2,\delta_1^2,\delta_1^2\delta_2)\\
    &w^{(4)} = (1,\delta_1,\delta_2,\delta_1^2,\delta_2^2,\delta_2^3)
\end{align*}

\[
N^{(1)}_1 =\left[
\begin{array}{cccccc}
    0 & 0  & 0 & 0 & 0 & 0  \\ 
    1 & 0  & 0 & 0 & 0 & 0 \\ 
    0 & 0 &  0&  0&  0&  0\\ 
    0 & 0 & 1 & 0 &  0 & 0  \\ 
    0 & 1 & 0 & 0 & 0 & 0  \\ 
    0 & 0 & 0 & 1 & -\frac{333}{100} &  0 \\ 
\end{array}
\right],\, N^{(1)}_2 =\left[
\begin{array}{cccccc}
    0 & 0  & 0 & 0 & 0 & 0  \\ 
    0 & 0  & 0 & 0 & 0 & 0 \\ 
    1 & 0  & 0 & 0 & 0 &  0\\ 
    0 & 1 & -\frac{3}{10} & 0 & 0 & 0  \\ 
    0 & 0 & 0 & 0 & 0 & 0  \\ 
    0 & 0 & 0 & -\frac{3}{10} & 1 &  0 \\ 
\end{array}
\right],
\]

The type is $\braket{III_0|IV_2|IV_1}$

\[
N^{(1)}_1 =\left[
\begin{array}{cccccc}
    0 & 0  & 0 & 0 & 0 & 0  \\ 
    1 & 0  & 0 & 0 & -\frac 89 & 0 \\ 
    0 & 0 &  0&  0&  -\frac 89&  0\\ 
    0 & 0 & 1 & 0 &  -2 & 0  \\ 
    0 & 1 & 0 & 0 & -2 & 0  \\ 
    0 & 0 & 0 & 1 & -1 &  0 \\ 
\end{array}
\right],\, N^{(1)}_2 =\left[
\begin{array}{cccccc}
    0 & 0  & 0 & 0 & 0 & 0  \\ 
    0 & 0  & 0 & 0 & 0 & 0 \\ 
    1 & 0  & 0 & 0 & 0 &  0\\ 
    0 & 1 & -\frac{3}{10} & 0 & 0 & 0  \\ 
    0 & 0 & 0 & 0 & 0 & 0  \\ 
    0 & 0 & 0 & -\frac{3}{10} & 1 &  0 \\ 
\end{array}
\right],
\]


We need to find a local basis such that the connection matrix has only first-order poles, and the residues are holomorphic at the origin. Denote the new basis as $w' = wg$, the gauge transformation formula is
\[
A_i\rightarrow g^{-1}A_ig+g^{-1}\nabla_{\partial_i}g,
\]
where $A_i$ is the connection matrices along $\partial_i$.


\subsubsection{Yukawa coupling and symplectic form}
The symplectic form $Q$ is determined by the intersection matrix $Q_{ij} = \int_{V}w_i\cup w_j$, which in turn is determined by the $n$-point functions
\[
K^{ij} :=\int_{V} 1\wedge \delta_1^i\delta_2^j, \quad i+j=n.
\]
When $n=3$, this is the so-called Yukawa couplings. Rewrite the Picard-Fuchs operators
\begin{align*}
     P_1:=& (1+z_1)\delta_1^3+3z_1\delta_1^2\delta_2+3z_1\delta_1\delta_2^2+z_1\delta_2^3+2z_1\delta_1^2+4z_1\delta_1\delta_2+2z_1\delta_2^2\\
    & +\frac{11}{9}z_1\delta_1+ \frac{11}{9}z_1\delta_2 +\frac29    z_1 \\
     P_2:= & (z_1 + z_2 + 1)\delta_1^2+(2z_1+2z_2-1)\delta_1\delta_2+(z_1 + z_2 + 1)\delta_2^2\\
     &+(z_1+z_2)\delta_1+(z_1+z_2)\delta_2+\frac29(z_1+z_2).
\end{align*}
Together with the Griffith transversality, from $\int_V1\wedge P_1 =0$ we get
\[
(1+z_1)K^{3,0}+3z_1K^{2,1}+3z_1K^{1,2}+z_1K^{0,3} = 0.
\]
Similarly, from $\int_V1\wedge\delta_i P_2=0$, $i=1,2$, we get
\begin{align*}
    &(z_1 + z_2 + 1)K^{3,0}+(2z_1+2z_2-1)K^{2,1}+(z_1 + z_2 + 1)K^{1,2} =0,\\
    &(z_1 + z_2 + 1)K^{2,1}+(2z_1+2z_2-1)K^{1,2}+(z_1 + z_2 + 1)K^{0,3} =0.
\end{align*}
Therefore, $K^{3,0}$ determines all the other Yukawa couplings. More precisely, we have
\begin{align*}
    K^{21} & = \frac{- 2z_1^2 - z_1z_2 - z_1 + z_2^2 + 2z_2 + 1}{3z_1(z_1 + z_2 - 2)}K^{30},\\
    K^{12} & = \frac{- 2z_2^2 - z_1z_2 - z_2 + z_1^2 + 2z_1 + 1}{3z_1(z_1 + z_2 - 2)}K^{30},\\
    K^{03} & = \frac{z_2}{z_1}K^{30}.
\end{align*}
We note these results are consistent with the $\bZ/2\bZ$ symmetry. Next, from $\int_V 1\wedge \delta_1 P_1=0$, we have
\begin{equation}\label{eqn5.4}
\begin{split}
0 = & (1+z_1)K^{4,0}+3z_1K^{3,1}+3z_1K^{2,2}+z_1K^{1,3}+3z_1K^{3,0}\\
& +7z_1K^{2,1}+5z_1K^{1,2}+z_1K^{0,3}, 
\end{split}
\end{equation}
similarly, from $\int_{V}1\wedge\delta_1^2P_2$, we have
\begin{equation}\label{eqn5.5}
\begin{split}
0 =  & (z_1+z_2+1)K^{4,0}+(2z_1+2z_2-1)K^{31}+(z_1+z_2+1)K^{2,2}\\
& + (3z_1+z_2)K^{3,0}+(5z_1+z_2)K^{2,1}+2z_1K^{1,2}.
\end{split}
\end{equation}

To simplify the notation, we denote $\braket{i,j|l,m}=\int_V\delta_1^i\delta_2^j\wedge \delta_1^l\delta_2^m$. Then $K^{i,j} = \braket{0,0|i,j}$, and we have $\braket{i,j|l,m} = -\braket{l,m|i,j}$. From $\delta_1^2K^{2,0}=0$, we have $K^{4,0} = -2\braket{1,0|3,0}$, and since $\delta_1K^{3,0} = \braket{1,0|3,0}+K^{4,0}$, we have $K^{4,0} = 2\delta_1K^{3,0}$. Similarly, from $\delta_1\delta_2K^{2,0}=\delta_1^2K^{1,1}=0$ we get
\begin{align*}
    &\braket{1,0|2,1}+\braket{0,1|3,0}+\braket{1,1|2,0}+K^{3,1} = 0,\\
    &2\braket{1,0|2,1}-\braket{1,1|2,0}+K^{3,1}=0.
\end{align*}
combining with
$\delta_1 K^{2,1} = \braket{1,0|2,1}+K^{3,1}$, and $\delta_2K^{3,0} = \braket{0,1|3,0}+K^{3,1}$, we have
\[
K^{3,1} = \frac{3}{2}\delta_1K^{2,1} +\frac12\delta_2K^{3,0}.
\]
By symmetry, we have
\[
K^{1,3} = \frac{3}{2}\delta_2K^{1,2} +\frac12\delta_1K^{0,3},\quad K^{0,4} = 2\delta_2K^{0,3}. 
\]
A similar calculation shows 
\[
K^{2,2} = \delta_1 K^{1,2}+\delta_2 K^{2,1},
\]
Then substitute everything back into \eqref{eqn5.4}, we arrive at the system of first order PDEs
\begin{equation}
    \begin{split}
        &\delta_1K^{3,0} = \frac{N_1}{(z_1+z_2-2)D_A}K^{3,0}\\
        &\delta_2K^{3,0} = \frac{N_2}{(z_1+z_2-2)D_A}K^{3,0}
    \end{split}
\end{equation}
where 
\begin{align*}
    N_1 = & - z_1^4 - 2z_1^3z_2 + 4z_1^3 - 18z_1^2z_2 + 9z_1^2 + 2z_1z_2^3 + 6z_1z_2^2  + 6z_1z_2 + 2z_1 \\
    & + z_2^4 + z_2^3 - 3z_2^2 - 5z_2 - 2,\\
    N_2 = & -z_2(2z_1^3 + 6z_1^2z_2 - 30z_1^2 + 6z_1z_2^2 - 6z_1z_2 + 42z_1  + 2z_2^3 \\
    & - 3z_2^2 - 12z_2 - 7),
\end{align*}
With the help of Wolfram Mathematica$^{{\text{\tiny\textregistered}}}$ we get
\[
K^{3,0} = \frac{cz_1}{(z_1+z_2-2)D_A},\quad c\neq 0,
\]
Next, the intersection matrix is given by
\begin{equation}
    Q = \left[\begin{array}{cccccc}
    0 & 0 & 0 & 0 & 0 & K^{2,1} \\
    0 & 0 & 0 & \braket{1,0|1,1} & \braket{1,0|2,0} & \braket{1,0|2,1} \\
    0 & 0 & 0 & \braket{0,1|1,1} & \braket{0,1|2,0} & \braket{0,1|2,1} \\
    * & * & * & 0 & \braket{1,1|2,0} & \braket{1,1|2,1} \\
    * & * & * & * & 0 & \braket{2,0|2,1} \\
    * & * & * & * & * & 0 \\
    \end{array}\right]
\end{equation}
where the $*$ entries are determined by the rest by the antisymmetricity of $Q$. By the previous calculation, we have
\begin{equation}
    Q = \left[\begin{array}{cccccc}
    0 & 0 & 0 & 0 & 0 & K^{2,1} \\
    0 & 0 & 0 & -K^{2,1} & -K^{3,0} & \delta_1K^{2,1}-K^{3,1} \\
    0 & 0 & 0 & -K^{1,2} & -K^{2,1} & \delta_2K^{2,1}-K^{2,2} \\
    * & * & * & 0 & 2\delta_1K^{2,1}-K^{3,1} & \braket{1,1|2,1} \\
    * & * & * & * & 0 & \braket{2,0|2,1} \\
    * & * & * & * & * & 0 \\
    \end{array}\right],
\end{equation}
Now, the entry $\braket{1,1|2,1}$ can be determined by the following. First, from
\begin{equation}
    \begin{aligned}
        0  = & \delta_1^3K^{3,0}  =  \braket{3,0|0,2}+3\braket{2,0|1,2}+3\braket{1,0|2,2}+K^{3,2},\\
        0  = &  \delta_1^2\delta_2K^{1,1}  =  \braket{2,1|1,1}+\braket{2,0|1,2}+2\braket{1,1|2,1}+2\braket{1,0|2,2}\\
        & +\braket{0,1|3,1} +K^{3,2}, \\
        \delta_1^2 K^{1,2} = & \braket{2,0|1,2}+ 2\braket{1,0|2,2}+K^{3,2},\\
        \delta_1\delta_2K^{2,1} = & \braket{1,1|2,1}+\braket{1,0|2,2}+\braket{0,1|3,1}+K^{3,2},\\
        \delta_2^2K^{3,0} = &\braket{0,2|3,0}+2\braket{0,1|3,1} + K^{3,2},
    \end{aligned}
\end{equation}
we get
\[
\braket{1,1|2,1} = K^{3,2}-\delta_1^2K^{1,2}  -\frac32\delta_1\delta_2K^{2,1}-\frac 12\delta_2^2 K^{3,0},
\]
and similarly one has
\begin{align*}
    \braket{2,0|2,1} = & K^{4,1}-\frac 43\delta_1K^{3,1}-\frac16\delta_2K^{4,0}\\
    = & K^{4,1} - 2 \delta_1^2K^{2,1}-\delta_1\delta_2K^{3,0}.
\end{align*}
Therefore, these two entries are determined by the 5-point functions $K^{3,2},K^{4,1}$. To calculate these 5-point functions, we consider $0 =\int_V1\wedge \delta_1^i\delta_2^j P_1$, $i+j=2$, and $0 =\int_V1\wedge \delta_1^i\delta_2^j P_2$, $i+j=3$. These 7 equations can be used to rewrite the 6 different 5-point functions into 4-point and 3-point functions. More precisely, the first 6 equations gives
\begin{align*}
    0 = & (z_1 + 1)K^{5,0} + 3z_1K^{4,1} + 4z_1K^{4,0} + 3z_1K^{3,2} + 10z_1K^{3,1} + (56z_1K^{3,0})/9 + z_1K^{2,3} \\ & + 8z_1K^{2,2} + (110z_1K^{2,1})/9 + 2z_1K^{1,3} + 7z_1K^{1,2} + z_1K^{0,3}\\
    0 = & (z_1 + 1)K^{4,1} + 3z_1K^{3,2} + 3z_1K^{3,1} + 3z_1K^{2,3} + 7z_1K^{2,2} + (29z_1K^{2,1})/9 + z_1K^{1,4} \\& + 5z_1K^{1,3} + (47z_1K^{1,2})/9 + z_1K^{0,4} + 2z_1K^{0,3}\\
    0 = & (z_1 + 1)K^{3,2} + 3z_1K^{2,3} + 2z_1K^{2,2} + 3z_1K^{1,4} + 4z_1K^{1,3} + (11z_1K^{1,2})/9 + z_1K^{0,5} \\ & + 2z_1K^{0,4} + (11z_1K^{0,3})/9\\
    0 = & (z_1 + z_2 + 1)K^{5,0} + (2z_1 + 2z_2 - 1)K^{4,1} + (4z_1 + z_2)K^{4,0} + (z_1 + z_2 + 1)K^{3,2} + (7z_1 + z_2)K^{3,1} \\ &+ ((56z_1)/9 + (2z_2)/9)K^{3,0} + 3z_1K^{2,2} + 9z_1K^{2,1} + 3z_1K^{1,2}\\
    0 = & (z_1 + z_2 + 1)K^{4,1} + z_2K^{4,0} + (2z_1 + 2z_2 - 1)K^{3,2} + (3z_1 + 3z_2)K^{3,1} + z_2K^{3,0} \\ & +(z_1 + z_2 + 1)K^{2,3} + (5z_1 + 2z_2)K^{2,2} + \frac{29z_1 + 11z_2}{9}K^{2,1} + 2z_1K^{1,3} + 4z_1K^{1,2} + z_1K^{0,3}\\
    0 = & (z_1 + z_2 + 1)K^{3,2} + 2z_2K^{3,1} + z_2K^{3,0} + (2z_1 + 2z_2 - 1)K^{2,3} + (2z_1 + 5z_2)K^{2,2} + 4z_2K^{2,1} \\ & + (z_1 + z_2 + 1)K^{1,4} + (3z_1 + 3z_2)K^{1,3} + ((11z_1)/9 + (29z_2)/9)K^{1,2} + z_1K^{0,4} + z_1K^{0,3}
\end{align*}
and from these equations we can solve $K^{4,1}$ and $K^{3,2}$, which in turn gives $\braket{1,1|2,1}$ and $\braket{2,0|2,1}$. The result is
\begin{align*}
\braket{1,1|2,1} & = -\frac{cz_1N_3}{27(z_1+z_2-2)^4D_A^2} ,\\
\braket{2,0|2,1} & =-\frac{cz_1N_4}{27(z_1+z_2-2)^4D_A^2},
\end{align*}
where $N_3,N_4\in \bZ[z_1,z_2]$ are two complicated degree 6 polynomials. Therefore, at $z_1=z_2=0$, the symplectic form is given by
\[
Q =\frac{c}{12}\cdot \left[
\begin{array}{cccccc}
    0 & 0  & 0 & 0 & 0 & 1  \\ 
    0 & 0  & 0 & -1 & 0 & 0 \\ 
    0 & 0 &  0&  -1&  -1&  0\\ 
    0 & 1 & 1 & 0 & 0 & 0  \\ 
    0 & 0 & 1 & 0 & 0 & 0  \\ 
    -1 & 0 & 0 & 0 & 0 &  0 \\ 
\end{array}
\right],
\]
By rescale the local basis $w$ by $\left(\frac{c}{12}\right)^{\frac12}$, we can get rid of the coefficient $\frac{c}{12}$. These calculations are done with the help of Matlab$^{{\text{\tiny\textregistered}}}$.


\subsubsection{Cohomology of $\bP_\Delta$}
Recall we have the correspondence between $\Xi$ and $T$-invariant divisors given by $v_i\leftrightarrow D_{v_i}$.  Further, recall $A_{3}(X_{\Sigma})$ is generated by the class of $T$-invariant divisors, so in what follows, we will use $D_{v_i}$ to denote either the $T$-invariant divisor, or its linear equivalence class or its cohomology class under Poincar{\'e} duality.
Associate to each $v_i$ a variable $x_i$ and consider the polynomial ring $\bZ[x_1,x_2,\cdots,x_6]$. Since $\bP_\Delta$ is smooth and complete, by Jurkiewicz-Danilov's theorem (see e.g. \cite{CLS11}), we have
$$
H^*(\bP_\Delta,\bZ) \cong \bZ[x_1,x_2\cdots,x_6]/(I_{RS}+J).
$$
The Stanley-Reisier ideal $I_{SR}$ is generated by the monomials $\prod_{i\in E}x_i$, as $E$ runs over all the subset of $\Delta$ such that $E$ does not form a cone in $\Sigma$. The Stanley-Reisier ideal 
can be read off from \eqref{eqn5.1}. We have
$$
I_{SR} = (x_1x_5x_6,x_2x_3x_4).
$$
The ideal $J$ is generated by $r_i\cdot \mathbf{x}$, $i=1,2,3,4$, where $r_i$ are the rows of $P$, and $\mathbf{x} = (x_1,x_2,\cdots,x_6)$. We have
$$
J = (x_1+x_5-2x_6,x_2-x_4+x_5-x_6,x_3-x_4+2x_5-2x_6,x_5-x_6),
$$
which gives the relations among classes
\begin{equation}\label{divrel}
D_{v_1} = D_{v_5} = D_{v_6}, \quad D_{v_2}=D_{v_3}=D_{v_4},
\end{equation}
Then we have
\begin{equation}\label{cohoXs}
H^*(X_\Sigma,\bZ)\cong \bZ[x_1,x_2\cdots,x_7]/(I_{RS}+J) \cong \bZ[x_1,x_2]/I'_{RS},
\end{equation}
where
$$
I'_{RS} = (x_1^3,x_2^3).
$$



\subsubsection{Local basis}
At the boundary point $D_{v_1^s}\cap E_3$, the residue in the basis $w$ is
\begin{align*}
&\widetilde N^{(1)}_1:=\tRes(\nabla^{(1)}_{\partial_s}) =\left[
\begin{array}{cccccc}
    0 & 0  & 2/3 & 0 & 0 & 0  \\ 
    1 & 0  & 3 & 2/3 & 0 & 0 \\ 
    0 & 0 &  3&  0&  0&  0\\ 
    0 & 0 & 10 & 3 &  0 & 0  \\ 
    0 & 1 & 0 & 3 & 0 & 2/3  \\ 
    0 & 0 & 0 & 10 & 0 &  3 \\ 
\end{array}
\right],\\
&\widetilde N^{(1)}_2:=\tRes(\nabla^{(2)}_{\partial_t}) =\left[
\begin{array}{cccccc}
    0 & 0  & -\frac29 & 0 & 0 & 0  \\ 
    0 & 0  & -1 & -\frac 29 & 0 & 0 \\ 
    1 & 0  & -1 & 0 & 0 &  0\\ 
    0 & 1 & -3 & -1 & 0 & 0  \\ 
    0 & 0 & 0 & -1 & 0 & -\frac29  \\ 
    0 & 0 & 0 & -3 & 0 &  -1 \\ 
\end{array}
\right].
\end{align*}
Since $[\widetilde N^{(1)}_1,\widetilde N^{(1)}_2]=0$, we can find their generalized multi-eigenvalues and multi-eigenvectors, the result is
\begin{align*}
    &\gamma_1 = (1,0,0,0,0,0)^t,\quad && \nu_1 = (0,0) && \text{order} = (3,3);\\
    &\gamma_2 = (0,1,0,0,0,0)^t,\quad && \nu_1 = (0,0);&& \text{order} = (2,2   );\\
    &\gamma_3 = (0,0,0,0,1,0)^t,\quad && \nu_1 = (0,0);&& \text{order} = (1,1   );\\
    &\gamma_4 = \gamma_5 =  (1,\frac32,\frac92,0,-\frac 92,0)^tt    ,\quad && \nu_1 = (0,-1);&& \text{order} = (3,1);\\
    &\gamma_5 = (0,1,0,\frac 92,\frac 32,0)^t ,\quad && \nu_1 = (0,-1);&& \text{order} = (2 ,1);\\
    &\gamma_6 = (0,0,0,0,1,\frac92          )^t,\quad && \nu_1 = (0,-1);&& \text{order} = (1,1);\\
\end{align*}
Now, we change the local basis to $\gamma:=(w\gamma_1,w\gamma_2,\dots,w\gamma_6)$, the residue of connection matrix then becomes lower triangle, with the diagonals  $(0,0,0,0,0,0)$ and $(0,0,0,-1,-1,-1)$, respectively. Then take a new local basis  \[
\gamma'=(w\gamma_1,w\gamma_2,w\gamma_3,tw\gamma_4,tw\gamma_5,tw\gamma_6),
\]
the residues become strictly lower triangular, and we have

\[
N^{(1)}_1 =\left[
\begin{array}{cccccc}
    0 & 0  & 0 & 0 & 0 & 0  \\ 
    1 & 0  & 0 & 0 & 0 & 0 \\ 
    0 & 1 &  0&  0&  0&  0\\ 
    0 & 0 & 0 & 0 &  0 & 0  \\ 
    0 & 0 & 0 & 1 & 0 & 0  \\ 
    0 & 0 & 0 & 0 & 1 &  0 \\ 
\end{array}
\right],\, N^{(1)}_2 =\left[
\begin{array}{cccccc}\
    0 & 0  & 0 & 0 & 0 & 0 \\ 
    3 & 0  & 0 & 0 &    0 &  0\\ 
    0 & 3 & 0 & 0 & 0 & 0  \\ 
    -\frac29 & 0 & 0 & 0 & 0 & 0  \\ 
    0 & -\frac29 & 0 & 0 & 0 &  0 \\ 
     0 & 0  & -\frac29 & 0 & 0 & 0  \\ 
\end{array}
\right],
\]
The type is $\braket{\mathrm{III_0}|IV_2|IV_1}$.

Similarly, the type at other boundary points can be calculated similarly. We have: $E_1\cap E_2$, the 


\subsubsection{The even cohomology of $\check V$}
By Baytrev mirror construction, the mirror of $V$ is the generic anti-canonical hypersurface $\check V\subset \bP_\Delta$. The anti-canonical class is $-K_{\bP_\Delta}= \sum_{i=1}^nD_{v_i} = 3D_{v_1}+3D_{v_2}$. In particular, since $-K_{\bP_\Delta}$ is ample, we know $D_{v_1}+D_{v_2}$ sits inside the K{\"a}hler cone.

First, by Lefschetz hyperplane theorem, we have
$$
i^*:H^2(\bP_\Delta,\bZ) \cong H^2(\check V,\bZ)\cong H^{1,1}(\check V,\bZ).
$$
Then $H^2(X,\bZ)$ is generated by $T_1:=i^*D_{v_1}, T_2:=i^*D_{v_2}$ as an abelian group. Next, since pullback preserves the K{\"a}hler cone, we have $T_1+T_2$ sitting inside the K{\"a}hler cone of $\check V$. By hard Lefschetz theorem, we have $(T_1+T_2)\cdot :H^2(X,\bQ)\rightarrow H^4(X,\bQ)$ is an isomorphism. Therefore, we have
$$
H^4(X,\bQ) = \bQ\braket{T_1(T_1+T_2),T_2(T_1+T_2)}.
$$
Now, we want to calculate the intersection numbers \[
\check I_{i,j} :=\int_{\check V}(T_{i}\cup T_j(T_1+T_2)),\quad i,j=1,2.
\]
By the projection formula, we have $I_{i,
j} = \int_{\bP_\Delta}3(D_{v_1}+D_{v_2})^2D_{v_i}D_{v_j} = 6-3\delta_{i,j}$. Where we have used the fact $\int_{\bP_\Delta} D_{v_1}^iD_{v_2}^j = \delta_{i,2}\delta_{j,2}$. In particular, we have $T_1T_2 = T_1^2+T_2^2$, and $T_1^2T_2 = T_1T_2^2$.


Next, since $\check V$ is smooth, the total Chern class $c(\check V)$ can be calculated by the normal sheaf sequence
\[
0\rightarrow \mathscr{T}_{\check V}\rightarrow i^*\mathscr{T}_{\bP_\Delta}\rightarrow i^*K_{\bP_\Delta}^{\otimes-1}\rightarrow 0,
\]
then
\begin{align*}
   c(\check V) & = \frac{i^*c(\bP_\Delta)}{i^*\cO(3D_{v_1}+3D_{v_2   })}= \frac{(1+T_1)^3(1+T_2)^3}{1+3(T_1+T_2)}\\
& = 1+3(T_1^2+3T_1T_2+T_2^2)-27(T_1^2T_2+T_1T_2^2) \\
& = 1+12T_1T_2-27(T_1^2T_2+T_1T_2^2)
\end{align*}
where $c(\bP_\Delta)$ is calculated by the toric Euler sequence
\[
0\rightarrow \Omega_{\bP_\Delta}^1\rightarrow \bigoplus _{i=1}^6 \mathcal{O}_{\bP_\Delta}(-D_{v_i})\rightarrow \mathrm{Pic}(\bP_{\Delta})\otimes \mathcal{O}_X\rightarrow 0.
\]
See chapter 13 of \cite{CLS11} for details. Then we have $c_2(\check V) = 3(T_1^2+3T_1T_2+T_2^2)$, and the total Todd class is $td(\check V) = 1+\frac{c_2(\check V)}{12} = 1+T_1T_2$.

Consider the following symplectic form on $K(\check V,\bQ):=K(\check V)\otimes\bQ$
\begin{align*}
   K(\check V,\bQ)\otimes K(\check V,\bQ) &\rightarrow \bQ \\
    E_1\otimes E_2&\rightarrow\chi(E_1,E_2) = \int_{\check V}ch(E_1^*)ch(E_2)td(\check V),
\end{align*}
where the last equality is given by the Hirzebruch-Riemann-Roch formula. 

Then we have a half-integral symplectic basis of $K(\check V,
bQ)$
\[
\{1 = E_1^{(0)}= [\cO_{\check V}],E_{1}^{(1)},E_{2}^{(1)},E_{2}^{(2)},E_{1}^{(2)},E_{1}^{(3)}\}
\]
where $E_{i}^{(m)}\in K(\check V,\bQ)$ supports on codimension $m$ cycle. Under the isomorphism $ch:K(\check V,\bQ)\rightarrow H^{even}(\check V,\bQ)$, their total Chern characteristics are
\[
\{1,(T_1-\sum_{l}\frac 12 C_{1l}K_l)td^{-1}_{\hat X_0},(T_2-\sum_{l}\frac 12 C_{2l}K_l)td^{-1}_{\hat X_0},K_2,K_1,V\} 
\]
where $K_1 = \frac{T_2^2}{3}$, $K_2 = \frac{T_1^2}{3}$ satisfies $\int_{\check 
V}T_iK_j = \delta_{i,j}$; $V = -\frac{T_1^2T_2+T_1T_2^2}{6}$, satisfies $\int_{\check V}V = -1$. The $C_{i,j}$ are some integers undetermined integers.

\subsubsection{Hosono's $w$-function}
The principal period can be read off from \eqref{susfan5.2}
\[
w = \sum_{n_1,n_2\geq0}\frac{\Gamma(3(n_1+n_2)+1)}{\Gamma(n_1+1)^3\Gamma(n_2+1)^3}z_1^{n_1}z_2^{n_2}.
\]

The Hosono's $w$-function is a $H^{even}(\check V,\bC)$-valued function on $\bar B$, that is closed related to the Givental's $I$-function, which in our case it is
\begin{equation}\label{wbasexpan}
\begin{split}
    w  = & w_0\cdot ch(E_1^{(0)})+ w_{1}^{(1)}\cdot ch(E_1^{(1)})+ w_1^{(2)}\cdot ch(E_1^{(2)})+ w_2^{(2)}ch(E_{2}^{(2)}) \\
    & + w_1^{(2)}\cdot ch(E_{1}^{(2)}) +w_3 \cdot ch(E_1^{(3)})\\
    = & w_0 + w_1^{(1)}T_1+w_2^{(1)}T_2+(w_1^{(2)}-\frac{C_{11}}{2}w_1^{(1)}-\frac{C_{21}}{2}w_2^{(1)})K_1\\
    & + (w_2^{(2)}- \frac{C_{12}}{2}w_1^{(1)}-\frac{C_{22}}{2}w_2^{(1)})K_2 + (3w_{1}^{(1)}+3w_{1}^{(1)}+w_3)V.
\end{split}
\end{equation}
Then we have
\begin{align*}
    &w_0 = w|_{T_i=0}, \quad w_1^{(1)}= \partial_{T_1}w|_{T_i=0},  \quad w_2^{(1)} = \partial_{T_2}w|_{T_i=0}, \\
    & w_2^{(2)} = \frac32 \partial_{T_1}^2w|_{T_i=0}+3\partial_{T_1}\partial_{T_2}w|_{T_i=0}+\frac{C_{12}}{2}\partial_{T_1}w|_{T_i=0}+\frac{C_{22}}{2}\partial_{T_2}w|_{T_i=0},\\
    & w_1^{(2)} = \frac32 \partial_{T_2}^2w|_{T_i=0}+3\partial_{T_1}\partial_{T_2}w|_{T_i=0}+\frac{C_{11}}{2}\partial_{T_1}w|_{T_i=0}+\frac{C_{21}}{2}\partial_{T_2}w|_{T_i=0},\\
    & w_3 = -\frac{3}{2}(\partial_{T_1}^2\partial_{T_2}w|_{T_i=0}+\partial_{T_1}\partial^2_{T_2}w|_{T_i=0}) - 3\partial_{T_1}w|_{T_i=0}-3\partial_{T_2}w|_{T_i=0}.
\end{align*}

The monodromy of these functions is given by
$$
\left[
\begin{array}{l}
     w_0\\
     w_1^{(1)}\\
     w_2^{(1)}\\
     w_2^{(2)}\\
     w_1^{(2)}\\
     w^{(3)}\\
\end{array}
\right] \xrightarrow{z_1\rightarrow e^{2\pi i}z_1} \left[
\begin{array}{ccccccc}
     1 & 0 & 0 & 0 & 0 & 0 \\
     1 & 1 & 0 & 0 & 0 & 0 \\
     0 & 0 & 1 & 0 & 0 & 0 \\
     \frac{C_{12}+3}{2} & 3 & 3 & 1 & 0 & 0\\
     \frac{C_{11}}{2} & 0 & 3  & 0 & 1 & 0\\
     -3 & \frac{C_{11}}{2}  & \frac{C_{21}-3}{2} & 0 & -1 & 1
\end{array}
\right]\cdot
\left[
\begin{array}{l}
     w_0\\
     w_1^{(1)}\\
     w_2^{(1)}\\
     w^{(3)}\\
     w_1^{(2)}\\
     w_2^{(2)}\\
\end{array}
\right],
$$
and
$$
\left[
\begin{array}{l}
     w_0\\
     w_1^{(1)}\\
     w_2^{(1)}\\
     w^{(3)}\\
     w_1^{(2)}\\
     w_2^{(2)}\\
\end{array}
\right] \xrightarrow{z_1\rightarrow e^{2\pi i}z_1} \left[
\begin{array}{ccccccc}
     1 & 0 & 0 & 0 & 0 & 0 \\
     0 & 1 & 0 & 0 & 0 & 0 \\
     1 & 0 & 1 & 0 & 0 & 0 \\
     \frac{C_{22}}{2} & 3 & 0 & 1 & 0 & 0\\ 
     \frac{C_{21}+3}{2} & 3 & 3 & 0 & 1 & 0\\
     -3 & \frac{C_{12}-3}{2} & \frac{C_{22}}{2} & -1 & 0 & 1
\end{array}
\right]\cdot
\left[
\begin{array}{l}
     w_0\\
     w_1^{(1)}\\
     w_2^{(1)}\\
     w^{(3)}\\
     w_1^{(2)}\\
     w_2^{(2)}\\
\end{array}
\right],
$$
Denote these two matrices as $S_1,S_2$. They are symplectic with respect to the standard symplectic
\begin{equation}\label{strdsympl}
Q^{st}:=\left[\begin{array}{cccccc}0 & 0 & 0 & 0 & 0 & -1 \\0 & 0 & 0 & 0 & -1 & 0 \\0 & 0 & 0 & -1 & 0 & 0 \\0 & 0 & 1 & 0 & 0 & 0 \\0 & 1 & 0 & 0 & 0 & 0 \\1 & 0 & 0 & 0 & 0 & 0\end{array}\right],
\end{equation}
we have $C_{12} = C_{21}$. As can be checked easily, these two monodromies are simply
\[
v\rightarrow S_i\cdot v = ch(\cO(-T_i))\cup v = e^{-T_i}\cup v,\quad \forall v\in H^{even}(\check V,\bQ).
\]



\subsection{$V_{(2,38)}$}
The toric data for              


The suspended toric data for $Int(\Delta^\circ)=\Xi$ is
\begin{equation}
\frac{\bar A}{\bar B}=
\begin{array}{c|ccccccc}
\bar\Xi& \bar v_1 & \bar v_2 & \bar v_3 &\bar  v_4 &\bar  v_5 &\bar  v_6 &\bar  v_7\\
\hline
\bar r_1 & 1 & 0 & 0 & 1 & -4 & -1 & 0\\
\bar r_2 & 0 & 1 & 0 & 2 & -5 & -1 & 0\\
\bar r_3 & 0 & 0 & 1 & 1 & -2 & 0 & 0\\
\bar r_4 & 0 & 0 & 0 & 3 & -3 & 0 & 0\\
\bar r_5 & 1 & 1 & 1 & 1 & 1 & 1 & 1\\
\hline
\bar w_1 & 1 & 1 & 0 & 0 & 0 & 1 & -3\\
\bar w_2 & 0 & 0 & 1 & 1 & 1 & -3 & 0
\end{array}.
\end{equation}


\subsubsection{Picard-Fuchs equation}
\begin{align*}
    & P_1 = \delta_1(\delta_1-3\delta_2) +3z_1(3\delta_1+1)(3\delta_1+2)\\
    & P_2 = \delta_2^3-z_2(\delta_1-3\delta_2)(\delta_1-3\delta_2-1)(\delta_1-3\delta_2-2)
\end{align*}
after a rescale, the Picard-Fuchs operators become
\begin{align*}
    & P_1 = \delta_1(\delta_1-3\delta_2) +z_1(\delta_1+\frac13)(\delta_1+\frac23)\\
    & P_2 = \delta_2^3-z_2(\frac13\delta_1-\delta_2)(\frac13\delta_1-\delta_2-\frac13)(\frac13\delta_1-\delta_2-\frac13)
\end{align*}
The singular locus contains inside
\[
D_A \cup  D_1 \cup D_{v_1^s}\cup D_{v_2^s}\cup D_{v_3^s}\cup D_{v_4^s}
\]
where $D_A = (1+z_1)^3+z_1^3z_2$, $D_1 = 1+z_2$.


==> Toric_geometry_and_mirror_symmetry.tex <==
% ---------------------------------------
\section{Toric geometry and mirror symmetry}\label{sec04}
%----------------------------------------

In this section, we fix the notations that will be used in the next section, these notations are standard and follow closely to those in \cite{CK99,CLS11}.

\subsection{Toric variety}
Denote the standard full-rank integral lattice group in $\bQ^n$ as $N$ and its dual lattice as $M$. 
We will use the $k\times k$ matrices $\frac{A_{n\times k}}{B_{(k-n)\times k}}$ to record the toric data. The column vectors of $A$ form a finite set 
\[
\{v_1,v_2,\dots,v_k\}=:\Xi\subset N,
\]
and the set of row vectors $\{w_1,w_2,\dots,w_{r}\}$ ($r := k-n$) of $B$ generates the lattice of relations among $\Xi$
\[
\Lambda:=\left\{l=(l_i)\in \bZ^k: \sum_{i=1}^k l_iv_i=0\right\}
\]
over $\bZ$. 
In particular, we have $A\cdot B^t=0$. These data can be viewed as recording either the information about a polyhedral fan $\Sigma$ or the information of an integral polytope $\Delta^\circ$. Each of these points of view leads to one way to construct a toric variety, which we now briefly review.

For a strongly convex rational polyhedral fan $\Sigma\subset N_\bR:=N\otimes_\bZ\bR$, denotes $\Sigma(m)$ as the set of its $m$-dimension cones. In this case, we use the columns of $A$ to record the primitive generators generators of elements in $\Sigma(1)$. Denote, $\sigma_{i_1,\dots,i_m}\in \Sigma(m)$ as the $m$-dimension cone that generated by $\{v_{i_1},v_{i_2},\dots,v_{i_m}\}$. 
The toric variety constructed from $\Sigma$ is denoted as $X_\Sigma$. More precisely, let $S = \bC[x_1,\dots,x_k]$, and recall
\begin{definition}[Cox ideal] The \textit{Cox ideal} $I_{\Sigma}$ is the ideal of $S$ generated by the monomials corresponding to each $\sigma\in\Sigma(n)$, defined by
\[
x_{i_1}x_{i_2}\dots x_{i_\alpha},\quad  \alpha = k-\sigma(1),\,\bR_+\cdot v_{i_s}\notin\sigma(1).
\]
\end{definition}
Then, we have 
\begin{align*}
X_\Sigma  & = \mathrm{Proj}_\Sigma(S)\\
& = [\mathrm{Spec(S)- \bV(I_\Sigma)}]\sslash G,
\end{align*}
where the $G:=(\bC^*)^r$-action on $\bC^k$ is determined by the matrix $B$ as
\begin{align*}
G\times \bC^k & \rightarrow  \bC^k\\
(s_1,\dots,s_r)\times(x_1,\dots,x_k) & \rightarrow \left(\prod_{i=1}^rs_i^{w_{i,1}}\cdot x_1,\cdots,\prod_{i=1}^rs_i^{w_{i,k}}\cdot x_k\right)
\end{align*}


Now, for an integral polytope $\Delta^\circ$ i.e., a polytope in $\bR^k$ whose vertices lies in $N$. The toric data records all the integral points inside the polytope $\Delta^\circ$, i.e., $\Xi=\Delta^\circ \cap N$. Denote the toric variety constructed from it as $\bP_{\Delta^\circ}$, which is the Zariski closure of the open immersion
\begin{align*}
    (\bC^*)^n &\hookrightarrow \bP^k\\
    (t_1,\dots,t_n)& \rightarrow \left[\prod_{i=1}^nt_i^{r_{1,i}}:\prod_{i=1}^nt_i^{r_{2,i}}:\cdots:\prod_{i=1}^nt_i^{r_{k,i}}\right].
\end{align*}


Each of the constructions contains a top dimensional Zariski dense tori $T:=(\bC^*)^n$ inside the toric variety. For $\bP_{\Delta^\circ}$ it is clear from the construction, whereas for $X_\Sigma$, we have $T = (\bC^*)^k/G\hookrightarrow X_{\Sigma}$.


\subsubsection{Reflexive polytope and Baytrev mirror}
The starting point of a Baytrev's mirror construction is a reflexive polytope and its mirror, we first recall some definitions.
\begin{definition}\label{defnf}
For an arbitrary full-dimensional integral polytope $\Delta\subset M_\bR$ of dimension $r$. For each codimension $s$ face $F$ of $\Delta$, let $\sigma_F$  be the $s$-dimensional strongly convex rational polyhedral cone in $N_\bR$ defined as
\[
\sigma_F:=\{v\in N_\bR|\braket{m,v}\geq\braket{m',v} ,\forall m\in F,m'\in \Delta\}.
\]
Then the \textit{normal fan} $\Sigma_\Delta$ of $\Delta$ is the union of all $\sigma_F$.      
\end{definition}

\begin{definition}\label{defref}
Let $\Delta$ be the same in Definition \ref{defnf}, then $\Delta\subset M_\bR$ is called \textit{reflexive} if for any codimension-1 face $\Gamma$, there is a unique vector $v_\Gamma\in N$, such that
$$
\Delta = \{m\in M_\bR|\braket{m,v_F}\geq-1,\forall F\}.
$$
and $\mathrm{Int}(\Delta) \cap N = \{0\}$.
\end{definition}




The \textit{polar dual} $\Delta^\circ\subset N_\bR$ of $\Delta$ is defined as
$$
\Delta^\circ:=\{n\in N_\bR|\braket{m,n}\geq -1, \forall m\in \Delta\},
$$
Now, if $\Delta$ is reflexive, $\Delta^\circ$ is also reflexive and we have $(\Delta^\circ)^\circ = \Delta$. Furthermore, $\Delta^\circ$ is the convex hull of $v_\Gamma$, and $\{v_\Gamma\}$ spans $\Sigma_\Delta(1)$.



By Baytrev mirror symmetry construction, the mirror of $X_\Sigma$, denote as $\check X_{\Sigma}$ is $\check X_{\Sigma}\cong X_{\Sigma^\circ}\cong \bP_{\Delta^\circ}$. On the level of the Calabi-Yau hypersurface, we have $\check X$ as the anti-canonical hypersurface of $\check X_{\Sigma}$ that is mirror to $X$.
The simplified moduli space of the complex structure of $\check X$ is also a toric variety whose normal fan is the secondary fan $\Sigma^s$.

\subsubsection{Automorphisms of $X_\Sigma$}
The automorphism group $\tAut(X_\Sigma)$ of $X_\Sigma$ is generated by three types of automorphisms that come from the $T$-action, the root symmetry, and the fan symmetry. The first two types of automorphism are continuous, together they generate the connected component $\tAut_0(X_\Sigma)$ of $\tAut(X_\Sigma)$.



The last type of automorphism comes from the symmetry of the $\Sigma$. More precisely, these automorphisms form a finite group $\tAut(\Sigma)$, the subgroup of $\tAut(N)$ that preserves $\Sigma$.

\subsubsection{Moduli space}
There are three moduli spaces that are naturally associated to $V$, i.e., the polynomial moduli, the simplified moduli, and the complex moduli. First, the polynomial moduli is
\[
\cM_{\mathrm{poly}} := \bP(L(\Delta^\circ\cap N))/\mathrm{Aut}(X_{\Sigma^\circ}),
\]
which parameterized the complex structure of $V$ that can be realized as hypersurfaces of $X_\Sigma$. The simplified is
\[
\cM_{\mathrm{simp}}:= \bP(L((\Delta^\circ\cap N))_0)/T,
\]
where $(\Delta^\circ\cap N))_0$ is the subset of $\Delta^\circ\cap N$ that excludes the points that lies in the interior of any facet of $\Delta^\circ$.

The \textit{dominance theorem} conjectured in \cite{AGM93} and proved in \cite{CK99} states that 
\begin{theorem}
    The quotient map $\phi:\cM_{\mathrm{simp}}\rightarrow \cM_{\mathrm{poly}}$ is generically {\'e}tale.
\end{theorem}
Apparently, the generic degree of $\phi$ is $|\mathrm{Aut}(\Sigma)|$. Finally, the complex moduli $\cM$ is the moduli space of the complex structure. $\cM$ and $\cM_{\mathrm{poly}}$ are related by the following proposition
\begin{proposition}
    
\end{proposition}







\subsection{GKZ system}

To construct the GKZ system $\tau(\bar A,\beta)$, we need to introduce 
the suspended fan $\bar\Sigma$ of $\Sigma$, whose 1-dimensional cones are generated by $\bar \Xi :=(\Xi\cup\{0\})\times 1$. The toric data of the suspended fan will be denoted as $\frac{\bar A}{\bar B}$. Then $\tau(\bar A,\beta)$ is the cyclic $\mathcal D_{\bC^{k+1}}-$module, determined by the left ideal $I_{GKZ}$ in Weyl algebra, which is generated by
\[
\prod_{l_i>0}\partial_{\lambda_i}^{l_i}-\prod_{l_j<0}\partial_{\lambda_j}^{l_j},\quad l\in\Lambda,
\]
and 
\[
\sum_{j=1}^{k+1}r_{i,j}\lambda_j\partial_j+\beta_i,\quad i=1,\dots,n+1,
\]
where $\lambda_i$ are the coordinates of $\bC^{k+1}$, and $\beta = (0,\dots,0,-1)$. Let $j:(\bC^*)^{k+1}\hookrightarrow \bC^{k+1}$ be the inclusion, then $j^*\tau(\bar A,\beta)$ 

The GKZ system can be viewed as a special case of the tautological system \cite{LSY13}. In that regard, the suspension corresponds to including the Euler operator in the system and is the only part specialized to the anti-canonical section.

\subsubsection{Principal A-determinant}
The singular locus of the GKZ system $\tau(\bar A,\beta)$.
